Tamed Warping Network for High-Resolution Semantic Video Segmentation

Recent approaches for fast semantic video segmentation have reduced redundancy by warping feature maps across adjacent frames, greatly speeding up the inference phase. However, the accuracy drops seriously owing to the errors incurred by warping. In this paper, we propose a novel framework and design a simple and effective correction stage after warping. Specifically, we build a non-key-frame CNN, fusing warped context features with current spatial details. Based on the feature fusion, our Context Feature Rectification~(CFR) module learns the model's difference from a per-frame model to correct the warped features. Furthermore, our Residual-Guided Attention~(RGA) module utilizes the residual maps in the compressed domain to help CRF focus on error-prone regions. Results on Cityscapes show that the accuracy significantly increases from $67.3\%$ to $71.6\%$, and the speed edges down from $65.5$ FPS to $61.8$ FPS at a resolution of $1024\times 2048$. For non-rigid categories, e.g., ``human'' and ``object'', the improvements are even higher than 18 percentage points.

==> __latexindent_temp.tex <==
Flownet2& 67.1			& - 		& 27.8 		 & - \\

==> abstract.tex <==
%%%%%%%%% ABSTRACT
\begin{abstract}

	Real-time semantic segmentation on high-resolution videos is challenging due to the strict requirements of speed. 
	Recent approaches have utilized the inter-frame continuity to reduce redundant computation by warping the feature maps across adjacent frames, greatly speeding up the inference phase. However, their accuracy drops significantly owing to the imprecise motion estimation and error accumulation.
%In this paper, we propose a novel architecture, named Warp-Refine Network~(WRNet), to bridge the performance gap between a warped model and a per-frame model. 
	In this paper, we propose a framework named Tamed Warping Network (TWNet) to introduce a simple and effective correction stage right after the warping stage, aiming to improve the accuracy and robustness of warping-based models. 
%Specifically, we design the context feature refinement~(CFR) module to refine the warped features with the help of per-frame model features. Furthermore, we introduce the residual-guided attention~(RGA) module to help CFR focus on error-prone regions. % distance  the residual in feature space.
	The experimental results on the Cityscapes dataset show that with the correction, the accuracy~(mIoU) significantly increases from $67.3\%$ to $71.6\%$, and the speed edges down from 65.5 FPS to 61.8 FPS. For non-rigid categories such as  ``human'' and ``object'', the improvements of IoU are even higher than 18 percentage points.
	%Futhormore, we introduce the residual-guided attention~(RGA) module to help CFR focus on rectifying regions with 
	% efficient refinement stage after interior feature warping.
	%Experimental results demonstrate that WRNet speeds up the per-frame segmentation network by $1.8\times$ while achieves comparable accuracy. %Also, we perform experiments to show the refinement stage is able to increase the robustness by alleviating the error accumulation problem. 
	%On the Cityscapes dataset, WRNet is able to achieve $71.6\%$ mIoU at $61.8$ FPS for $1024\times 2048$ inputs. %without any rescaling. 
	%A high-speed version achieves $69.5\%$ mIoU at $84.9$ FPS. %To the best of our knowledge, both these two versions the faster all the state-of-the-art real-time approaches.

	\keywords{Semantic Video Segmentation, Feature Correction, Warping, Real-Time}

\end{abstract}

	


==> appliedsciences-twnet/Definitions/journalnames.tex <==
%%Updated on 9 May 2023
%,% Website Name,%,%,% Website Name,%%,% Full Name,%%,% Short Name,%%,% DOI abbr,%%,% ISSN,% \continuouspages
%\DeclareOption{}{\gdef\@journal{}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{acoustics}{\gdef\@journal{acoustics}\gdef\@journalfull{Acoustics}\gdef\@journalshort{Acoustics}\gdef\@doiabbr{acoustics}\gdef\@ISSN{2624-599X}\gdef\@continuouspages{yes}}
\DeclareOption{actuators}{\gdef\@journal{actuators}\gdef\@journalfull{Actuators}\gdef\@journalshort{Actuators}\gdef\@doiabbr{act}\gdef\@ISSN{2076-0825}}
\DeclareOption{addictions}{\gdef\@journal{addictions}\gdef\@journalfull{Addictions}\gdef\@journalshort{Addictions}\gdef\@doiabbr{}\gdef\@ISSN{0006-0006}}
\DeclareOption{admsci}{\gdef\@journal{admsci}\gdef\@journalfull{Administrative Sciences}\gdef\@journalshort{Adm. Sci.}\gdef\@doiabbr{admsci}\gdef\@ISSN{2076-3387}}
\DeclareOption{adolescents}{\gdef\@journal{adolescents}\gdef\@journalfull{Adolescents}\gdef\@journalshort{Adolescents}\gdef\@doiabbr{adolescents}\gdef\@ISSN{2673-7051}\gdef\@continuouspages{yes}}
\DeclareOption{aerobiology}{\gdef\@journal{aerobiology}\gdef\@journalfull{Aerobiology}\gdef\@journalshort{Aerobiology}\gdef\@doiabbr{aerobiology}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{aerospace}{\gdef\@journal{aerospace}\gdef\@journalfull{Aerospace}\gdef\@journalshort{Aerospace}\gdef\@doiabbr{aerospace}\gdef\@ISSN{2226-4310}}
\DeclareOption{agriculture}{\gdef\@journal{agriculture}\gdef\@journalfull{Agriculture}\gdef\@journalshort{Agriculture}\gdef\@doiabbr{agriculture}\gdef\@ISSN{2077-0472}}
\DeclareOption{agriengineering}{\gdef\@journal{agriengineering}\gdef\@journalfull{AgriEngineering}\gdef\@journalshort{AgriEngineering}\gdef\@doiabbr{agriengineering}\gdef\@ISSN{2624-7402}\gdef\@continuouspages{yes}}
\DeclareOption{agrochemicals}{\gdef\@journal{agrochemicals}\gdef\@journalfull{Agrochemicals}\gdef\@journalshort{Agrochemicals}\gdef\@doiabbr{agrochemicals}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{agronomy}{\gdef\@journal{agronomy}\gdef\@journalfull{Agronomy}\gdef\@journalshort{Agronomy}\gdef\@doiabbr{agronomy}\gdef\@ISSN{2073-4395}}
\DeclareOption{ai}{\gdef\@journal{ai}\gdef\@journalfull{AI}\gdef\@journalshort{AI}\gdef\@doiabbr{ai}\gdef\@ISSN{2673-2688}\gdef\@continuouspages{yes}}
\DeclareOption{air}{\gdef\@journal{air}\gdef\@journalfull{Air}\gdef\@journalshort{Air}\gdef\@doiabbr{air}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{algorithms}{\gdef\@journal{algorithms}\gdef\@journalfull{Algorithms}\gdef\@journalshort{Algorithms}\gdef\@doiabbr{a}\gdef\@ISSN{1999-4893}}
\DeclareOption{allergies}{\gdef\@journal{allergies}\gdef\@journalfull{Allergies}\gdef\@journalshort{Allergies}\gdef\@doiabbr{allergies}\gdef\@ISSN{2313-5786}}
\DeclareOption{alloys}{\gdef\@journal{alloys}\gdef\@journalfull{Alloys}\gdef\@journalshort{Alloys}\gdef\@doiabbr{alloys}\gdef\@ISSN{2674-063X}\gdef\@continuouspages{yes}}
\DeclareOption{analytica}{\gdef\@journal{analytica}\gdef\@journalfull{Analytica}\gdef\@journalshort{Analytica}\gdef\@doiabbr{analytica}\gdef\@ISSN{2673-4532}\gdef\@continuouspages{yes}}
\DeclareOption{analytics}{\gdef\@journal{analytics}\gdef\@journalfull{Analytics}\gdef\@journalshort{Analytics}\gdef\@doiabbr{analytics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{anatomia}{\gdef\@journal{anatomia}\gdef\@journalfull{Anatomia}\gdef\@journalshort{Anatomia}\gdef\@doiabbr{anatomia}\gdef\@ISSN{2813-0545}\gdef\@continuouspages{yes}}
\DeclareOption{anesthres}{\gdef\@journal{anesthres}\gdef\@journalfull{Anesthesia Research}\gdef\@journalshort{Anesth. Res.}\gdef\@doiabbr{anesthres}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{animals}{\gdef\@journal{animals}\gdef\@journalfull{Animals}\gdef\@journalshort{Animals}\gdef\@doiabbr{ani}\gdef\@ISSN{2076-2615}}
\DeclareOption{antibiotics}{\gdef\@journal{antibiotics}\gdef\@journalfull{Antibiotics}\gdef\@journalshort{Antibiotics}\gdef\@doiabbr{antibiotics}\gdef\@ISSN{2079-6382}}
\DeclareOption{antibodies}{\gdef\@journal{antibodies}\gdef\@journalfull{Antibodies}\gdef\@journalshort{Antibodies}\gdef\@doiabbr{antib}\gdef\@ISSN{2073-4468}}
\DeclareOption{antioxidants}{\gdef\@journal{antioxidants}\gdef\@journalfull{Antioxidants}\gdef\@journalshort{Antioxidants}\gdef\@doiabbr{antiox}\gdef\@ISSN{2076-3921}}
\DeclareOption{applbiosci}{\gdef\@journal{applbiosci}\gdef\@journalfull{Applied Biosciences}\gdef\@journalshort{Appl. Biosci.}\gdef\@doiabbr{applbiosci}\gdef\@ISSN{2813-0464}\gdef\@continuouspages{yes}}
\DeclareOption{appliedchem}{\gdef\@journal{appliedchem}\gdef\@journalfull{AppliedChem}\gdef\@journalshort{AppliedChem}\gdef\@doiabbr{appliedchem}\gdef\@ISSN{2673-9623}\gdef\@continuouspages{yes}}
\DeclareOption{appliedmath}{\gdef\@journal{appliedmath}\gdef\@journalfull{AppliedMath}\gdef\@journalshort{AppliedMath}\gdef\@doiabbr{appliedmath}\gdef\@ISSN{2673-9909}\gdef\@continuouspages{yes}}
\DeclareOption{applmech}{\gdef\@journal{applmech}\gdef\@journalfull{Applied Mechanics}\gdef\@journalshort{Appl. Mech.}\gdef\@doiabbr{applmech}\gdef\@ISSN{2673-3161}\gdef\@continuouspages{yes}}
\DeclareOption{applmicrobiol}{\gdef\@journal{applmicrobiol}\gdef\@journalfull{Applied Microbiology}\gdef\@journalshort{Appl. Microbiol.}\gdef\@doiabbr{applmicrobiol}\gdef\@ISSN{2673-8007}\gdef\@continuouspages{yes}}
\DeclareOption{applnano}{\gdef\@journal{applnano}\gdef\@journalfull{Applied Nano}\gdef\@journalshort{Appl. Nano}\gdef\@doiabbr{applnano}\gdef\@ISSN{2673-3501}\gdef\@continuouspages{yes}}
\DeclareOption{applsci}{\gdef\@journal{applsci}\gdef\@journalfull{Applied Sciences}\gdef\@journalshort{Appl. Sci.}\gdef\@doiabbr{app}\gdef\@ISSN{2076-3417}}
\DeclareOption{aquacj}{\gdef\@journal{aquacj}\gdef\@journalfull{Aquaculture Journal}\gdef\@journalshort{Aquac. J.}\gdef\@doiabbr{aquacj}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{architecture}{\gdef\@journal{architecture}\gdef\@journalfull{Architecture}\gdef\@journalshort{Architecture}\gdef\@doiabbr{architecture}\gdef\@ISSN{2673-8945}\gdef\@continuouspages{yes}}
\DeclareOption{arm}{\gdef\@journal{arm}\gdef\@journalfull{Advances in Respiratory Medicine}\gdef\@journalshort{Adv. Respir. Med.}\gdef\@doiabbr{arm}\gdef\@ISSN{2543-6031}\gdef\@continuouspages{yes}}
\DeclareOption{arthropoda}{\gdef\@journal{arthropoda}\gdef\@journalfull{Arthropoda}\gdef\@journalshort{Arthropoda}\gdef\@doiabbr{arthropoda}\gdef\@ISSN{2813-3323}\gdef\@continuouspages{yes}}
\DeclareOption{arts}{\gdef\@journal{arts}\gdef\@journalfull{Arts}\gdef\@journalshort{Arts}\gdef\@doiabbr{arts}\gdef\@ISSN{2076-0752}}
\DeclareOption{asc}{\gdef\@journal{asc}\gdef\@journalfull{Automatic Systems and Control}\gdef\@journalshort{Autom. Syst. Control}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{asi}{\gdef\@journal{asi}\gdef\@journalfull{Applied System Innovation}\gdef\@journalshort{Appl. Syst. Innov.}\gdef\@doiabbr{asi}\gdef\@ISSN{2571-5577}}
\DeclareOption{astronomy}{\gdef\@journal{astronomy}\gdef\@journalfull{Astronomy}\gdef\@journalshort{Astronomy}\gdef\@doiabbr{astronomy}\gdef\@ISSN{2674-0346}\gdef\@continuouspages{yes}}
\DeclareOption{atmosphere}{\gdef\@journal{atmosphere}\gdef\@journalfull{Atmosphere}\gdef\@journalshort{Atmosphere}\gdef\@doiabbr{atmos}\gdef\@ISSN{2073-4433}}
\DeclareOption{atoms}{\gdef\@journal{atoms}\gdef\@journalfull{Atoms}\gdef\@journalshort{Atoms}\gdef\@doiabbr{atoms}\gdef\@ISSN{2218-2004}}
\DeclareOption{audiolres}{\gdef\@journal{audiolres}\gdef\@journalfull{Audiology Research}\gdef\@journalshort{Audiol. Res.}\gdef\@doiabbr{audiolres}\gdef\@ISSN{2039-4349}\gdef\@continuouspages{yes}}
\DeclareOption{automation}{\gdef\@journal{automation}\gdef\@journalfull{Automation}\gdef\@journalshort{Automation}\gdef\@doiabbr{automation}\gdef\@ISSN{2673-4052}\gdef\@continuouspages{yes}}
\DeclareOption{axioms}{\gdef\@journal{axioms}\gdef\@journalfull{Axioms}\gdef\@journalshort{Axioms}\gdef\@doiabbr{axioms}\gdef\@ISSN{2075-1680}}
\DeclareOption{bacteria}{\gdef\@journal{bacteria}\gdef\@journalfull{Bacteria}\gdef\@journalshort{Bacteria}\gdef\@doiabbr{bacteria}\gdef\@ISSN{2674-1334}\gdef\@continuouspages{yes}}
\DeclareOption{batteries}{\gdef\@journal{batteries}\gdef\@journalfull{Batteries}\gdef\@journalshort{Batteries}\gdef\@doiabbr{batteries}\gdef\@ISSN{2313-0105}}
\DeclareOption{bdcc}{\gdef\@journal{bdcc}\gdef\@journalfull{Big Data and Cognitive Computing}\gdef\@journalshort{Big Data Cogn. Comput.}\gdef\@doiabbr{bdcc}\gdef\@ISSN{2504-2289}}
\DeclareOption{behavsci}{\gdef\@journal{behavsci}\gdef\@journalfull{Behavioral Sciences}\gdef\@journalshort{Behav. Sci.}\gdef\@doiabbr{bs}\gdef\@ISSN{2076-328X}}
\DeclareOption{beverages}{\gdef\@journal{beverages}\gdef\@journalfull{Beverages}\gdef\@journalshort{Beverages}\gdef\@doiabbr{beverages}\gdef\@ISSN{2306-5710}}
\DeclareOption{biochem}{\gdef\@journal{biochem}\gdef\@journalfull{BioChem}\gdef\@journalshort{BioChem}\gdef\@doiabbr{biochem}\gdef\@ISSN{2673-6411}\gdef\@continuouspages{yes}}
\DeclareOption{bioengineering}{\gdef\@journal{bioengineering}\gdef\@journalfull{Bioengineering}\gdef\@journalshort{Bioengineering}\gdef\@doiabbr{bioengineering}\gdef\@ISSN{2306-5354}}
\DeclareOption{biologics}{\gdef\@journal{biologics}\gdef\@journalfull{Biologics}\gdef\@journalshort{Biologics}\gdef\@doiabbr{biologics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biology}{\gdef\@journal{biology}\gdef\@journalfull{Biology}\gdef\@journalshort{Biology}\gdef\@doiabbr{biology}\gdef\@ISSN{2079-7737}}
\DeclareOption{biomass}{\gdef\@journal{biomass}\gdef\@journalfull{Biomass}\gdef\@journalshort{Biomass}\gdef\@doiabbr{biomass}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biomechanics}{\gdef\@journal{biomechanics}\gdef\@journalfull{Biomechanics}\gdef\@journalshort{Biomechanics}\gdef\@doiabbr{biomechanics}\gdef\@ISSN{2673-7078}\gdef\@continuouspages{yes}}
\DeclareOption{biomed}{\gdef\@journal{biomed}\gdef\@journalfull{BioMed}\gdef\@journalshort{BioMed}\gdef\@doiabbr{biomed}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biomedicines}{\gdef\@journal{biomedicines}\gdef\@journalfull{Biomedicines}\gdef\@journalshort{Biomedicines}\gdef\@doiabbr{biomedicines}\gdef\@ISSN{2227-9059}}
\DeclareOption{biomedinformatics}{\gdef\@journal{biomedinformatics}\gdef\@journalfull{BioMedInformatics}\gdef\@journalshort{BioMedInformatics}\gdef\@doiabbr{biomedinformatics}\gdef\@ISSN{2673-7426}\gdef\@continuouspages{yes}}
\DeclareOption{biomimetics}{\gdef\@journal{biomimetics}\gdef\@journalfull{Biomimetics}\gdef\@journalshort{Biomimetics}\gdef\@doiabbr{biomimetics}\gdef\@ISSN{2313-7673}}
\DeclareOption{biomolecules}{\gdef\@journal{biomolecules}\gdef\@journalfull{Biomolecules}\gdef\@journalshort{Biomolecules}\gdef\@doiabbr{biom}\gdef\@ISSN{2218-273X}}
\DeclareOption{biophysica}{\gdef\@journal{biophysica}\gdef\@journalfull{Biophysica}\gdef\@journalshort{Biophysica}\gdef\@doiabbr{biophysica}\gdef\@ISSN{2673-4125}\gdef\@continuouspages{yes}}
\DeclareOption{biosensors}{\gdef\@journal{biosensors}\gdef\@journalfull{Biosensors}\gdef\@journalshort{Biosensors}\gdef\@doiabbr{bios}\gdef\@ISSN{2079-6374}}
\DeclareOption{biotech}{\gdef\@journal{biotech}\gdef\@journalfull{BioTech}\gdef\@journalshort{BioTech}\gdef\@doiabbr{biotech}\gdef\@ISSN{2673-6284}}
\DeclareOption{birds}{\gdef\@journal{birds}\gdef\@journalfull{Birds}\gdef\@journalshort{Birds}\gdef\@doiabbr{birds}\gdef\@ISSN{2673-6004}\gdef\@continuouspages{yes}}
\DeclareOption{blockchains}{\gdef\@journal{blockchains}\gdef\@journalfull{Blockchains}\gdef\@journalshort{Blockchains}\gdef\@doiabbr{blockchains}\gdef\@ISSN{2813-5288}\gdef\@continuouspages{yes}}
\DeclareOption{bloods}{\gdef\@journal{bloods}\gdef\@journalfull{Bloods}\gdef\@journalshort{Bloods}\gdef\@doiabbr{bloods}\gdef\@ISSN{2673-415X}}
\DeclareOption{blsf}{\gdef\@journal{blsf}\gdef\@journalfull{Biology and Life Sciences Forum}\gdef\@journalshort{Biol. Life Sci. Forum}\gdef\@doiabbr{blsf	}\gdef\@ISSN{2673-9976}}
\DeclareOption{brainsci}{\gdef\@journal{brainsci}\gdef\@journalfull{Brain Sciences}\gdef\@journalshort{Brain Sci.}\gdef\@doiabbr{brainsci}\gdef\@ISSN{2076-3425}}
\DeclareOption{breath}{\gdef\@journal{breath}\gdef\@journalfull{Breath}\gdef\@journalshort{Breath}\gdef\@doiabbr{breath}\gdef\@ISSN{}}
\DeclareOption{buildings}{\gdef\@journal{buildings}\gdef\@journalfull{Buildings}\gdef\@journalshort{Buildings}\gdef\@doiabbr{buildings}\gdef\@ISSN{2075-5309}}
\DeclareOption{businesses}{\gdef\@journal{businesses}\gdef\@journalfull{Businesses}\gdef\@journalshort{Businesses}\gdef\@doiabbr{businesses}\gdef\@ISSN{2673-7116}\gdef\@continuouspages{yes}}
\DeclareOption{cancers}{\gdef\@journal{cancers}\gdef\@journalfull{Cancers}\gdef\@journalshort{Cancers}\gdef\@doiabbr{cancers}\gdef\@ISSN{2072-6694}}
\DeclareOption{carbon}{\gdef\@journal{carbon}\gdef\@journalfull{C}\gdef\@journalshort{C}\gdef\@doiabbr{c}\gdef\@ISSN{2311-5629}}
\DeclareOption{cardiogenetics}{\gdef\@journal{cardiogenetics}\gdef\@journalfull{Cardiogenetics}\gdef\@journalshort{Cardiogenetics}\gdef\@doiabbr{cardiogenetics}\gdef\@ISSN{2035-8148}\gdef\@continuouspages{yes}}
\DeclareOption{catalysts}{\gdef\@journal{catalysts}\gdef\@journalfull{Catalysts}\gdef\@journalshort{Catalysts}\gdef\@doiabbr{catal}\gdef\@ISSN{2073-4344}}
\DeclareOption{cells}{\gdef\@journal{cells}\gdef\@journalfull{Cells}\gdef\@journalshort{Cells}\gdef\@doiabbr{cells}\gdef\@ISSN{2073-4409}}
\DeclareOption{ceramics}{\gdef\@journal{ceramics}\gdef\@journalfull{Ceramics}\gdef\@journalshort{Ceramics}\gdef\@doiabbr{ceramics}\gdef\@ISSN{2571-6131}\gdef\@continuouspages{yes}}
\DeclareOption{challenges}{\gdef\@journal{challenges}\gdef\@journalfull{Challenges}\gdef\@journalshort{Challenges}\gdef\@doiabbr{challe}\gdef\@ISSN{2078-1547}}
\DeclareOption{chemengineering}{\gdef\@journal{chemengineering}\gdef\@journalfull{ChemEngineering}\gdef\@journalshort{ChemEngineering}\gdef\@doiabbr{chemengineering}\gdef\@ISSN{2305-7084}}
\DeclareOption{chemistry}{\gdef\@journal{chemistry}\gdef\@journalfull{Chemistry}\gdef\@journalshort{Chemistry}\gdef\@doiabbr{chemistry}\gdef\@ISSN{2624-8549}\gdef\@continuouspages{yes}}
\DeclareOption{chemosensors}{\gdef\@journal{chemosensors}\gdef\@journalfull{Chemosensors}\gdef\@journalshort{Chemosensors}\gdef\@doiabbr{chemosensors}\gdef\@ISSN{2227-9040}}
\DeclareOption{chemproc}{\gdef\@journal{chemproc}\gdef\@journalfull{Chemistry Proceedings}\gdef\@journalshort{Chem. Proc.}\gdef\@doiabbr{chemproc}\gdef\@ISSN{2673-4583}}
\DeclareOption{children}{\gdef\@journal{children}\gdef\@journalfull{Children}\gdef\@journalshort{Children}\gdef\@doiabbr{children}\gdef\@ISSN{2227-9067}}
\DeclareOption{chips}{\gdef\@journal{chips}\gdef\@journalfull{Chips}\gdef\@journalshort{Chips}\gdef\@doiabbr{chips}\gdef\@ISSN{2674-0710}\gdef\@continuouspages{yes}}
\DeclareOption{cimb}{\gdef\@journal{cimb}\gdef\@journalfull{Current Issues in Molecular Biology}\gdef\@journalshort{Curr. Issues Mol. Biol.}\gdef\@doiabbr{cimb}\gdef\@ISSN{1467-3045}\gdef\@continuouspages{yes}}
\DeclareOption{civileng}{\gdef\@journal{civileng}\gdef\@journalfull{CivilEng}\gdef\@journalshort{CivilEng}\gdef\@doiabbr{civileng}\gdef\@ISSN{2673-4109}\gdef\@continuouspages{yes}}
\DeclareOption{cleantechnol}{\gdef\@journal{cleantechnol}\gdef\@journalfull{Clean Technologies}\gdef\@journalshort{Clean Technol.}\gdef\@doiabbr{cleantechnol}\gdef\@ISSN{2571-8797}\gdef\@continuouspages{yes}}
\DeclareOption{climate}{\gdef\@journal{climate}\gdef\@journalfull{Climate}\gdef\@journalshort{Climate}\gdef\@doiabbr{cli}\gdef\@ISSN{2225-1154}}
\DeclareOption{clinpract}{\gdef\@journal{clinpract}\gdef\@journalfull{Clinics and Practice}\gdef\@journalshort{Clin. Pract.}\gdef\@doiabbr{clinpract}\gdef\@ISSN{2039-7283}\gdef\@continuouspages{yes}}
\DeclareOption{clockssleep}{\gdef\@journal{clockssleep}\gdef\@journalfull{Clocks \& Sleep}\gdef\@journalshort{Clocks\&Sleep}\gdef\@doiabbr{clockssleep}\gdef\@ISSN{2624-5175}\gdef\@continuouspages{yes}}
\DeclareOption{cmd}{\gdef\@journal{cmd}\gdef\@journalfull{Corrosion and Materials Degradation}\gdef\@journalshort{Corros. Mater. Degrad.}\gdef\@doiabbr{cmd}\gdef\@ISSN{2624-5558}\gdef\@continuouspages{yes}}
\DeclareOption{coasts}{\gdef\@journal{coasts}\gdef\@journalfull{Coasts}\gdef\@journalshort{Coasts}\gdef\@doiabbr{coasts}\gdef\@ISSN{2673-964X}\gdef\@continuouspages{yes}}
\DeclareOption{coatings}{\gdef\@journal{coatings}\gdef\@journalfull{Coatings}\gdef\@journalshort{Coatings}\gdef\@doiabbr{coatings}\gdef\@ISSN{2079-6412}}
\DeclareOption{colloids}{\gdef\@journal{colloids}\gdef\@journalfull{Colloids and Interfaces}\gdef\@journalshort{Colloids Interfaces}\gdef\@doiabbr{colloids}\gdef\@ISSN{2504-5377}}
\DeclareOption{colorants}{\gdef\@journal{colorants}\gdef\@journalfull{Colorants}\gdef\@journalshort{Colorants}\gdef\@doiabbr{colorants}\gdef\@ISSN{2079-6447}\gdef\@continuouspages{yes}}
\DeclareOption{commodities}{\gdef\@journal{commodities}\gdef\@journalfull{Commodities}\gdef\@journalshort{Commodities}\gdef\@doiabbr{commodities}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{compounds}{\gdef\@journal{compounds}\gdef\@journalfull{Compounds}\gdef\@journalshort{Compounds}\gdef\@doiabbr{compounds}\gdef\@ISSN{2673-6918}\gdef\@continuouspages{yes}}
\DeclareOption{computation}{\gdef\@journal{computation}\gdef\@journalfull{Computation}\gdef\@journalshort{Computation}\gdef\@doiabbr{computation}\gdef\@ISSN{2079-3197}}
\DeclareOption{computers}{\gdef\@journal{computers}\gdef\@journalfull{Computers}\gdef\@journalshort{Computers}\gdef\@doiabbr{computers}\gdef\@ISSN{2073-431X}}
\DeclareOption{condensedmatter}{\gdef\@journal{condensedmatter}\gdef\@journalfull{Condensed Matter}\gdef\@journalshort{Condens. Matter}\gdef\@doiabbr{condmat}\gdef\@ISSN{2410-3896}}
\DeclareOption{conservation}{\gdef\@journal{conservation}\gdef\@journalfull{Conservation}\gdef\@journalshort{Conservation}\gdef\@doiabbr{conservation}\gdef\@ISSN{2673-7159}\gdef\@continuouspages{yes}}
\DeclareOption{constrmater}{\gdef\@journal{constrmater}\gdef\@journalfull{Construction Materials}\gdef\@journalshort{Constr. Mater.}\gdef\@doiabbr{constrmater}\gdef\@ISSN{2673-7108}\gdef\@continuouspages{yes}}
\DeclareOption{cosmetics}{\gdef\@journal{cosmetics}\gdef\@journalfull{Cosmetics}\gdef\@journalshort{Cosmetics}\gdef\@doiabbr{cosmetics}\gdef\@ISSN{2079-9284}}
\DeclareOption{covid}{\gdef\@journal{covid}\gdef\@journalfull{COVID}\gdef\@journalshort{COVID}\gdef\@doiabbr{covid}\gdef\@ISSN{2673-8112}\gdef\@continuouspages{yes}}
\DeclareOption{crops}{\gdef\@journal{crops}\gdef\@journalfull{Crops}\gdef\@journalshort{Crops}\gdef\@doiabbr{crops}\gdef\@ISSN{2673-7655}\gdef\@continuouspages{yes}}
\DeclareOption{cryptography}{\gdef\@journal{cryptography}\gdef\@journalfull{Cryptography}\gdef\@journalshort{Cryptography}\gdef\@doiabbr{cryptography}\gdef\@ISSN{2410-387X}}
\DeclareOption{crystals}{\gdef\@journal{crystals}\gdef\@journalfull{Crystals}\gdef\@journalshort{Crystals}\gdef\@doiabbr{cryst}\gdef\@ISSN{2073-4352}}
\DeclareOption{csmf}{\gdef\@journal{csmf}\gdef\@journalfull{Computer Sciences \& Mathematics Forum}\gdef\@journalshort{Comput. Sci. Math. Forum}\gdef\@doiabbr{csmf}\gdef\@ISSN{2813-0324}}
\DeclareOption{ctn}{\gdef\@journal{ctn}\gdef\@journalfull{Clinical and Translational Neuroscience}\gdef\@journalshort{Clin. Transl. Neurosci.}\gdef\@doiabbr{ctn}\gdef\@ISSN{2514-183X}}
\DeclareOption{curroncol}{\gdef\@journal{curroncol}\gdef\@journalfull{Current Oncology}\gdef\@journalshort{Curr. Oncol.}\gdef\@doiabbr{curroncol}\gdef\@ISSN{1718-7729}\gdef\@continuouspages{yes}}
\DeclareOption{cyber}{\gdef\@journal{cyber}\gdef\@journalfull{Cyber}\gdef\@journalshort{Cyber}\gdef\@doiabbr{cyber}\gdef\@ISSN{2624-800X}}
\DeclareOption{dairy}{\gdef\@journal{dairy}\gdef\@journalfull{Dairy}\gdef\@journalshort{Dairy}\gdef\@doiabbr{dairy}\gdef\@ISSN{2624-862X}\gdef\@continuouspages{yes}}
\DeclareOption{data}{\gdef\@journal{data}\gdef\@journalfull{Data}\gdef\@journalshort{Data}\gdef\@doiabbr{data}\gdef\@ISSN{2306-5729}}
\DeclareOption{ddc}{\gdef\@journal{ddc}\gdef\@journalfull{Drugs and Drug Candidates}\gdef\@journalshort{Drugs Drug Candidates}\gdef\@doiabbr{ddc}\gdef\@ISSN{2813-2998}\gdef\@continuouspages{yes}}
\DeclareOption{dentistry}{\gdef\@journal{dentistry}\gdef\@journalfull{Dentistry Journal}\gdef\@journalshort{Dent. J.}\gdef\@doiabbr{dj}\gdef\@ISSN{2304-6767}}
\DeclareOption{dermato}{\gdef\@journal{dermato}\gdef\@journalfull{Dermato}\gdef\@journalshort{Dermato}\gdef\@doiabbr{dermato}\gdef\@ISSN{2673-6179}\gdef\@continuouspages{yes}}
\DeclareOption{dermatopathology}{\gdef\@journal{dermatopathology}\gdef\@journalfull{Dermatopathology}\gdef\@journalshort{Dermatopathology}\gdef\@doiabbr{dermatopathology}\gdef\@ISSN{2296-3529}\gdef\@continuouspages{yes}}
\DeclareOption{designs}{\gdef\@journal{designs}\gdef\@journalfull{Designs}\gdef\@journalshort{Designs}\gdef\@doiabbr{designs}\gdef\@ISSN{2411-9660}}
\DeclareOption{devices}{\gdef\@journal{devices}\gdef\@journalfull{Devices}\gdef\@journalshort{Devices}\gdef\@doiabbr{devices}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{diabetology}{\gdef\@journal{diabetology}\gdef\@journalfull{Diabetology}\gdef\@journalshort{Diabetology}\gdef\@doiabbr{diabetology}\gdef\@ISSN{2673-4540}\gdef\@continuouspages{yes}}
\DeclareOption{diagnostics}{\gdef\@journal{diagnostics}\gdef\@journalfull{Diagnostics}\gdef\@journalshort{Diagnostics}\gdef\@doiabbr{diagnostics}\gdef\@ISSN{2075-4418}}
\DeclareOption{dietetics}{\gdef\@journal{dietetics}\gdef\@journalfull{Dietetics}\gdef\@journalshort{Dietetics}\gdef\@doiabbr{dietetics}\gdef\@ISSN{2674-0311}\gdef\@continuouspages{yes}}
\DeclareOption{digital}{\gdef\@journal{digital}\gdef\@journalfull{Digital}\gdef\@journalshort{Digital}\gdef\@doiabbr{digital}\gdef\@ISSN{2673-6470}\gdef\@continuouspages{yes}}
\DeclareOption{disabilities}{\gdef\@journal{disabilities}\gdef\@journalfull{Disabilities}\gdef\@journalshort{Disabilities}\gdef\@doiabbr{disabilities}\gdef\@ISSN{2673-7272}\gdef\@continuouspages{yes}}
\DeclareOption{diseases}{\gdef\@journal{diseases}\gdef\@journalfull{Diseases}\gdef\@journalshort{Diseases}\gdef\@doiabbr{diseases}\gdef\@ISSN{2079-9721}}
\DeclareOption{diversity}{\gdef\@journal{diversity}\gdef\@journalfull{Diversity}\gdef\@journalshort{Diversity}\gdef\@doiabbr{d}\gdef\@ISSN{1424-2818}}
\DeclareOption{dna}{\gdef\@journal{dna}\gdef\@journalfull{DNA}\gdef\@journalshort{DNA}\gdef\@doiabbr{dna}\gdef\@ISSN{2673-8856}\gdef\@continuouspages{yes}}
\DeclareOption{drones}{\gdef\@journal{drones}\gdef\@journalfull{Drones}\gdef\@journalshort{Drones}\gdef\@doiabbr{drones}\gdef\@ISSN{2504-446X}}
\DeclareOption{dynamics}{\gdef\@journal{dynamics}\gdef\@journalfull{Dynamics}\gdef\@journalshort{Dynamics}\gdef\@doiabbr{dynamics}\gdef\@ISSN{2673-8716}\gdef\@continuouspages{yes}}
\DeclareOption{earth}{\gdef\@journal{earth}\gdef\@journalfull{Earth}\gdef\@journalshort{Earth}\gdef\@doiabbr{earth}\gdef\@ISSN{2673-4834}\gdef\@continuouspages{yes}}
\DeclareOption{ebj}{\gdef\@journal{ebj}\gdef\@journalfull{European Burn Journal}\gdef\@journalshort{Eur. Burn J.}\gdef\@doiabbr{ebj}\gdef\@ISSN{2673-1991}\gdef\@continuouspages{yes}}
\DeclareOption{ecm}{\gdef\@journal{ecm}\gdef\@journalfull{Emergency Care and Medicine}\gdef\@journalshort{Emerg. Care Med.}\gdef\@doiabbr{ecm}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{ecologies}{\gdef\@journal{ecologies}\gdef\@journalfull{Ecologies}\gdef\@journalshort{Ecologies}\gdef\@doiabbr{ecologies}\gdef\@ISSN{2673-4133}\gdef\@continuouspages{yes}}
\DeclareOption{econometrics}{\gdef\@journal{econometrics}\gdef\@journalfull{Econometrics}\gdef\@journalshort{Econometrics}\gdef\@doiabbr{econometrics}\gdef\@ISSN{2225-1146}}
\DeclareOption{economies}{\gdef\@journal{economies}\gdef\@journalfull{Economies}\gdef\@journalshort{Economies}\gdef\@doiabbr{economies}\gdef\@ISSN{2227-7099}}
\DeclareOption{education}{\gdef\@journal{education}\gdef\@journalfull{Education Sciences}\gdef\@journalshort{Educ. Sci.}\gdef\@doiabbr{educsci}\gdef\@ISSN{2227-7102}}
\DeclareOption{ejihpe}{\gdef\@journal{ejihpe}\gdef\@journalfull{European Journal of Investigation in Health, Psychology and Education}\gdef\@journalshort{Eur. J. Investig. Health Psychol. Educ.}\gdef\@doiabbr{ejihpe}\gdef\@ISSN{2254-9625}\gdef\@continuouspages{yes}}
\DeclareOption{electricity}{\gdef\@journal{electricity}\gdef\@journalfull{Electricity}\gdef\@journalshort{Electricity}\gdef\@doiabbr{electricity}\gdef\@ISSN{2673-4826}\gdef\@continuouspages{yes}}
\DeclareOption{electrochem}{\gdef\@journal{electrochem}\gdef\@journalfull{Electrochem}\gdef\@journalshort{Electrochem}\gdef\@doiabbr{electrochem}\gdef\@ISSN{2673-3293}\gdef\@continuouspages{yes}}
\DeclareOption{electronicmat}{\gdef\@journal{electronicmat}\gdef\@journalfull{Electronic Materials}\gdef\@journalshort{Electron. Mater.}\gdef\@doiabbr{electronicmat}\gdef\@ISSN{2673-3978}\gdef\@continuouspages{yes}}
\DeclareOption{electronics}{\gdef\@journal{electronics}\gdef\@journalfull{Electronics}\gdef\@journalshort{Electronics}\gdef\@doiabbr{electronics}\gdef\@ISSN{2079-9292}}
\DeclareOption{encyclopedia}{\gdef\@journal{encyclopedia}\gdef\@journalfull{Encyclopedia}\gdef\@journalshort{Encyclopedia}\gdef\@doiabbr{encyclopedia}\gdef\@ISSN{2673-8392}\gdef\@continuouspages{yes}}
\DeclareOption{endocrines}{\gdef\@journal{endocrines}\gdef\@journalfull{Endocrines}\gdef\@journalshort{Endocrines}\gdef\@doiabbr{endocrines}\gdef\@ISSN{2673-396X}\gdef\@continuouspages{yes}}
\DeclareOption{energies}{\gdef\@journal{energies}\gdef\@journalfull{Energies}\gdef\@journalshort{Energies}\gdef\@doiabbr{en}\gdef\@ISSN{1996-1073}}
\DeclareOption{eng}{\gdef\@journal{eng}\gdef\@journalfull{Eng}\gdef\@journalshort{Eng}\gdef\@doiabbr{eng}\gdef\@ISSN{2673-4117}\gdef\@continuouspages{yes}}
\DeclareOption{engproc}{\gdef\@journal{engproc}\gdef\@journalfull{Engineering Proceedings}\gdef\@journalshort{Eng. Proc.}\gdef\@doiabbr{engproc}\gdef\@ISSN{2673-4591}}
%\DeclareOption{ent}{\gdef\@journal{ent}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{entomology}{\gdef\@journal{entomology}\gdef\@journalfull{Entomology}\gdef\@journalshort{Entomology}\gdef\@doiabbr{entomology}\gdef\@ISSN{2813-0502}\gdef\@continuouspages{yes}}	
\DeclareOption{entropy}{\gdef\@journal{entropy}\gdef\@journalfull{Entropy}\gdef\@journalshort{Entropy}\gdef\@doiabbr{e}\gdef\@ISSN{1099-4300}}
\DeclareOption{environments}{\gdef\@journal{environments}\gdef\@journalfull{Environments}\gdef\@journalshort{Environments}\gdef\@doiabbr{environments}\gdef\@ISSN{2076-3298}}
\DeclareOption{environsciproc}{\gdef\@journal{environsciproc}\gdef\@journalfull{Environmental Sciences Proceedings}\gdef\@journalshort{Environ. Sci. Proc.}\gdef\@doiabbr{environsciproc}\gdef\@ISSN{2673-4931}}
\DeclareOption{epidemiologia}{\gdef\@journal{epidemiologia}\gdef\@journalfull{Epidemiologia}\gdef\@journalshort{Epidemiologia}\gdef\@doiabbr{epidemiologia}\gdef\@ISSN{2673-3986}\gdef\@continuouspages{yes}}
\DeclareOption{epigenomes}{\gdef\@journal{epigenomes}\gdef\@journalfull{Epigenomes}\gdef\@journalshort{Epigenomes}\gdef\@doiabbr{epigenomes}\gdef\@ISSN{2075-4655}}
\DeclareOption{est}{\gdef\@journal{est}\gdef\@journalfull{Electrochemical Science and Technology}\gdef\@journalshort{Electrochem. Sci. Technol.}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{fermentation}{\gdef\@journal{fermentation}\gdef\@journalfull{Fermentation}\gdef\@journalshort{Fermentation}\gdef\@doiabbr{fermentation}\gdef\@ISSN{2311-5637}}
\DeclareOption{fibers}{\gdef\@journal{fibers}\gdef\@journalfull{Fibers}\gdef\@journalshort{Fibers}\gdef\@doiabbr{fib}\gdef\@ISSN{2079-6439}}
\DeclareOption{fintech}{\gdef\@journal{fintech}\gdef\@journalfull{FinTech}\gdef\@journalshort{FinTech}\gdef\@doiabbr{fintech}\gdef\@ISSN{2674-1032}\gdef\@continuouspages{yes}}
\DeclareOption{fire}{\gdef\@journal{fire}\gdef\@journalfull{Fire}\gdef\@journalshort{Fire}\gdef\@doiabbr{fire}\gdef\@ISSN{2571-6255}}
\DeclareOption{fishes}{\gdef\@journal{fishes}\gdef\@journalfull{Fishes}\gdef\@journalshort{Fishes}\gdef\@doiabbr{fishes}\gdef\@ISSN{2410-3888}}
\DeclareOption{fluids}{\gdef\@journal{fluids}\gdef\@journalfull{Fluids}\gdef\@journalshort{Fluids}\gdef\@doiabbr{fluids}\gdef\@ISSN{2311-5521}}
\DeclareOption{foods}{\gdef\@journal{foods}\gdef\@journalfull{Foods}\gdef\@journalshort{Foods}\gdef\@doiabbr{foods}\gdef\@ISSN{2304-8158}}
\DeclareOption{forecasting}{\gdef\@journal{forecasting}\gdef\@journalfull{Forecasting}\gdef\@journalshort{Forecasting}\gdef\@doiabbr{forecast}\gdef\@ISSN{2571-9394}\gdef\@continuouspages{yes}}
\DeclareOption{forensicsci}{\gdef\@journal{forensicsci}\gdef\@journalfull{Forensic Sciences}\gdef\@journalshort{Forensic Sci.}\gdef\@doiabbr{forensicsci}\gdef\@ISSN{2673-6756}\gdef\@continuouspages{yes}}
\DeclareOption{forests}{\gdef\@journal{forests}\gdef\@journalfull{Forests}\gdef\@journalshort{Forests}\gdef\@doiabbr{f}\gdef\@ISSN{1999-4907}}
\DeclareOption{fossils}{\gdef\@journal{fossils}\gdef\@journalfull{Fossils}\gdef\@journalshort{Fossils}\gdef\@doiabbr{fossils}\gdef\@ISSN{2813-6284}\gdef\@continuouspages{yes}}
\DeclareOption{foundations}{\gdef\@journal{foundations}\gdef\@journalfull{Foundations}\gdef\@journalshort{Foundations}\gdef\@doiabbr{foundations}\gdef\@ISSN{2673-9321}\gdef\@continuouspages{yes}}
\DeclareOption{fractalfract}{\gdef\@journal{fractalfract}\gdef\@journalfull{Fractal and Fractional}\gdef\@journalshort{Fractal Fract.}\gdef\@doiabbr{fractalfract}\gdef\@ISSN{2504-3110}}
\DeclareOption{fuels}{\gdef\@journal{fuels}\gdef\@journalfull{Fuels}\gdef\@journalshort{Fuels}\gdef\@doiabbr{fuels}\gdef\@ISSN{2673-3994}\gdef\@continuouspages{yes}}
\DeclareOption{future}{\gdef\@journal{future}\gdef\@journalfull{Future}\gdef\@journalshort{Future}\gdef\@doiabbr{future}\gdef\@ISSN{2813-2882}\gdef\@continuouspages{yes}}
\DeclareOption{futureinternet}{\gdef\@journal{futureinternet}\gdef\@journalfull{Future Internet}\gdef\@journalshort{Future Internet}\gdef\@doiabbr{fi}\gdef\@ISSN{1999-5903}}
%\DeclareOption{futureparasites}{\gdef\@journal{futureparasites}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{futurepharmacol}{\gdef\@journal{futurepharmacol}\gdef\@journalfull{Future Pharmacology}\gdef\@journalshort{Future Pharmacol.}\gdef\@doiabbr{futurepharmacol}\gdef\@ISSN{2673-9879}\gdef\@continuouspages{yes}}
\DeclareOption{futurephys}{\gdef\@journal{futurephys}\gdef\@journalfull{Future Physics}\gdef\@journalshort{Future Phys.}\gdef\@doiabbr{futurephys}\gdef\@ISSN{2624-6503}}
\DeclareOption{futuretransp}{\gdef\@journal{futuretransp}\gdef\@journalfull{Future Transportation}\gdef\@journalshort{Future Transp.}\gdef\@doiabbr{futuretransp}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{galaxies}{\gdef\@journal{galaxies}\gdef\@journalfull{Galaxies}\gdef\@journalshort{Galaxies}\gdef\@doiabbr{galaxies}\gdef\@ISSN{2075-4434}}
\DeclareOption{games}{\gdef\@journal{games}\gdef\@journalfull{Games}\gdef\@journalshort{Games}\gdef\@doiabbr{g}\gdef\@ISSN{2073-4336}}
\DeclareOption{gases}{\gdef\@journal{gases}\gdef\@journalfull{Gases}\gdef\@journalshort{Gases}\gdef\@doiabbr{gases}\gdef\@ISSN{2673-5628}\gdef\@continuouspages{yes}}
\DeclareOption{gastroent}{\gdef\@journal{gastroent}\gdef\@journalfull{Gastroenterology Insights}\gdef\@journalshort{Gastroenterol. Insights}\gdef\@doiabbr{gastroent}\gdef\@ISSN{2036-7422}\gdef\@continuouspages{yes}}
\DeclareOption{gastrointestdisord}{\gdef\@journal{gastrointestdisord}\gdef\@journalfull{Gastrointestinal Disorders}\gdef\@journalshort{Gastrointest. Disord.}\gdef\@doiabbr{gidisord}\gdef\@ISSN{2624-5647}\gdef\@continuouspages{yes}}
\DeclareOption{gastronomy}{\gdef\@journal{gastronomy}\gdef\@journalfull{Gastronomy}\gdef\@journalshort{Gastronomy}\gdef\@doiabbr{gastronomy}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{gels}{\gdef\@journal{gels}\gdef\@journalfull{Gels}\gdef\@journalshort{Gels}\gdef\@doiabbr{gels}\gdef\@ISSN{2310-2861}}
\DeclareOption{genealogy}{\gdef\@journal{genealogy}\gdef\@journalfull{Genealogy}\gdef\@journalshort{Genealogy}\gdef\@doiabbr{genealogy}\gdef\@ISSN{2313-5778}}
\DeclareOption{genes}{\gdef\@journal{genes}\gdef\@journalfull{Genes}\gdef\@journalshort{Genes}\gdef\@doiabbr{genes}\gdef\@ISSN{2073-4425}}
\DeclareOption{geographies}{\gdef\@journal{geographies}\gdef\@journalfull{Geographies}\gdef\@journalshort{Geographies}\gdef\@doiabbr{geographies}\gdef\@ISSN{2673-7086}\gdef\@continuouspages{yes}}
\DeclareOption{geohazards}{\gdef\@journal{geohazards}\gdef\@journalfull{GeoHazards}\gdef\@journalshort{GeoHazards}\gdef\@doiabbr{geohazards}\gdef\@ISSN{2624-795X}\gdef\@continuouspages{yes}}
\DeclareOption{geomatics}{\gdef\@journal{geomatics}\gdef\@journalfull{Geomatics}\gdef\@journalshort{Geomatics}\gdef\@doiabbr{geomatics}\gdef\@ISSN{2673-7418}\gdef\@continuouspages{yes}}
\DeclareOption{geosciences}{\gdef\@journal{geosciences}\gdef\@journalfull{Geosciences}\gdef\@journalshort{Geosciences}\gdef\@doiabbr{geosciences}\gdef\@ISSN{2076-3263}}
\DeclareOption{geotechnics}{\gdef\@journal{geotechnics}\gdef\@journalfull{Geotechnics}\gdef\@journalshort{Geotechnics}\gdef\@doiabbr{geotechnics}\gdef\@ISSN{2673-7094}\gdef\@continuouspages{yes}}
\DeclareOption{geriatrics}{\gdef\@journal{geriatrics}\gdef\@journalfull{Geriatrics}\gdef\@journalshort{Geriatrics}\gdef\@doiabbr{geriatrics}\gdef\@ISSN{2308-3417}}
\DeclareOption{grasses}{\gdef\@journal{grasses}\gdef\@journalfull{Grasses}\gdef\@journalshort{Grasses}\gdef\@doiabbr{grasses}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{gucdd}{\gdef\@journal{gucdd}\gdef\@journalfull{Gout, Urate, and Crystal Deposition Disease}\gdef\@journalshort{Gout Urate Cryst. Depos. Dis.}\gdef\@doiabbr{gucdd}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{hardware}{\gdef\@journal{hardware}\gdef\@journalfull{Hardware}\gdef\@journalshort{Hardware}\gdef\@doiabbr{hardware}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{hazardousmatters}{\gdef\@journal{hazardousmatters}\gdef\@journalfull{Hazardous Matters}\gdef\@journalshort{Hazard. Matters}\gdef\@doiabbr{}\gdef\@ISSN{0014-0014}}
\DeclareOption{healthcare}{\gdef\@journal{healthcare}\gdef\@journalfull{Healthcare}\gdef\@journalshort{Healthcare}\gdef\@doiabbr{healthcare}\gdef\@ISSN{2227-9032}}
\DeclareOption{hearts}{\gdef\@journal{hearts}\gdef\@journalfull{Hearts}\gdef\@journalshort{Hearts}\gdef\@doiabbr{hearts}\gdef\@ISSN{2673-3846}\gdef\@continuouspages{yes}}
\DeclareOption{hemato}{\gdef\@journal{hemato}\gdef\@journalfull{Hemato}\gdef\@journalshort{Hemato}\gdef\@doiabbr{hemato}\gdef\@ISSN{2673-6357}\gdef\@continuouspages{yes}}
\DeclareOption{hematolrep}{\gdef\@journal{hematolrep}\gdef\@journalfull{Hematology Reports}\gdef\@journalshort{Hematol. Rep.}\gdef\@doiabbr{hematolrep}\gdef\@ISSN{2038-8330}\gdef\@continuouspages{yes}}
\DeclareOption{heritage}{\gdef\@journal{heritage}\gdef\@journalfull{Heritage}\gdef\@journalshort{Heritage}\gdef\@doiabbr{heritage}\gdef\@ISSN{2571-9408}\gdef\@continuouspages{yes}}
\DeclareOption{higheredu}{\gdef\@journal{higheredu}\gdef\@journalfull{Trends in Higher Education}\gdef\@journalshort{Trends High. Educ.}\gdef\@doiabbr{higheredu}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{highthroughput}{\gdef\@journal{highthroughput}\gdef\@journalfull{High-Throughput}\gdef\@journalshort{High-Throughput}\gdef\@doiabbr{ht}\gdef\@ISSN{2571-5135}}
\DeclareOption{histories}{\gdef\@journal{histories}\gdef\@journalfull{Histories}\gdef\@journalshort{Histories}\gdef\@doiabbr{histories}\gdef\@ISSN{2409-9252}\gdef\@continuouspages{yes}}
\DeclareOption{horticulturae}{\gdef\@journal{horticulturae}\gdef\@journalfull{Horticulturae}\gdef\@journalshort{Horticulturae}\gdef\@doiabbr{horticulturae}\gdef\@ISSN{2311-7524}}
\DeclareOption{hospitals}{\gdef\@journal{hospitals}\gdef\@journalfull{Hospitals}\gdef\@journalshort{Hospitals}\gdef\@doiabbr{hospitals}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{humanities}{\gdef\@journal{humanities}\gdef\@journalfull{Humanities}\gdef\@journalshort{Humanities}\gdef\@doiabbr{h}\gdef\@ISSN{2076-0787}}
\DeclareOption{humans}{\gdef\@journal{humans}\gdef\@journalfull{Humans}\gdef\@journalshort{Humans}\gdef\@doiabbr{humans}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{hydrobiology}{\gdef\@journal{hydrobiology}\gdef\@journalfull{Hydrobiology}\gdef\@journalshort{Hydrobiology	}\gdef\@doiabbr{hydrobiology}\gdef\@ISSN{2673-9917}\gdef\@continuouspages{yes}}
\DeclareOption{hydrogen}{\gdef\@journal{hydrogen}\gdef\@journalfull{Hydrogen}\gdef\@journalshort{Hydrogen}\gdef\@doiabbr{hydrogen}\gdef\@ISSN{2673-4141}\gdef\@continuouspages{yes}}
\DeclareOption{hydrology}{\gdef\@journal{hydrology}\gdef\@journalfull{Hydrology}\gdef\@journalshort{Hydrology}\gdef\@doiabbr{hydrology}\gdef\@ISSN{2306-5338}}
\DeclareOption{hygiene}{\gdef\@journal{hygiene}\gdef\@journalfull{Hygiene}\gdef\@journalshort{Hygiene}\gdef\@doiabbr{hygiene}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{ice}{\gdef\@journal{ice}\gdef\@journalfull{Ice}\gdef\@journalshort{Ice}\gdef\@doiabbr{ice}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{idr}{\gdef\@journal{idr}\gdef\@journalfull{Infectious Disease Reports}\gdef\@journalshort{Infect. Dis. Rep.}\gdef\@doiabbr{idr}\gdef\@ISSN{2036-7449}\gdef\@continuouspages{yes}}
\DeclareOption{ijerph}{\gdef\@journal{ijerph}\gdef\@journalfull{International Journal of Environmental Research and Public Health}\gdef\@journalshort{Int. J. Environ. Res. Public Health}\gdef\@doiabbr{ijerph}\gdef\@ISSN{1660-4601}}
\DeclareOption{ijfs}{\gdef\@journal{ijfs}\gdef\@journalfull{International Journal of Financial Studies}\gdef\@journalshort{Int. J. Financial Stud.}\gdef\@doiabbr{ijfs}\gdef\@ISSN{2227-7072}}
\DeclareOption{ijgi}{\gdef\@journal{ijgi}\gdef\@journalfull{ISPRS International Journal of Geo-Information}\gdef\@journalshort{ISPRS Int. J. Geo-Inf.}\gdef\@doiabbr{ijgi}\gdef\@ISSN{2220-9964}}
\DeclareOption{ijms}{\gdef\@journal{ijms}\gdef\@journalfull{International Journal of Molecular Sciences}\gdef\@journalshort{Int. J. Mol. Sci.}\gdef\@doiabbr{ijms}\gdef\@ISSN{1422-0067}}
\DeclareOption{ijns}{\gdef\@journal{ijns}\gdef\@journalfull{International Journal of Neonatal Screening}\gdef\@journalshort{Int. J. Neonatal Screen.}\gdef\@doiabbr{ijns}\gdef\@ISSN{2409-515X}}
\DeclareOption{ijpb}{\gdef\@journal{ijpb}\gdef\@journalfull{International Journal of Plant Biology}\gdef\@journalshort{Int. J. Plant Biol.}\gdef\@doiabbr{ijpb}\gdef\@ISSN{2037-0164}\gdef\@continuouspages{yes}}
\DeclareOption{ijtm}{\gdef\@journal{ijtm}\gdef\@journalfull{International Journal of Translational Medicine}\gdef\@journalshort{Int. J. Transl. Med.}\gdef\@doiabbr{ijtm}\gdef\@ISSN{2673-8937}\gdef\@continuouspages{yes}}
\DeclareOption{ijtpp}{\gdef\@journal{ijtpp}\gdef\@journalfull{International Journal of Turbomachinery, Propulsion and Power}\gdef\@journalshort{Int. J. Turbomach. Propuls. Power}\gdef\@doiabbr{ijtpp}\gdef\@ISSN{2504-186X}}
\DeclareOption{ime}{\gdef\@journal{ime}\gdef\@journalfull{International Medical Education}\gdef\@journalshort{Int. Med. Educ.}\gdef\@doiabbr{ime}\gdef\@ISSN{2813-141X}\gdef\@continuouspages{yes}}
\DeclareOption{immuno}{\gdef\@journal{immuno}\gdef\@journalfull{Immuno}\gdef\@journalshort{Immuno}\gdef\@doiabbr{immuno}\gdef\@ISSN{2673-5601}\gdef\@continuouspages{yes}}
\DeclareOption{informatics}{\gdef\@journal{informatics}\gdef\@journalfull{Informatics}\gdef\@journalshort{Informatics}\gdef\@doiabbr{informatics}\gdef\@ISSN{2227-9709}}
\DeclareOption{information}{\gdef\@journal{information}\gdef\@journalfull{Information}\gdef\@journalshort{Information}\gdef\@doiabbr{info}\gdef\@ISSN{2078-2489}}
\DeclareOption{infrastructures}{\gdef\@journal{infrastructures}\gdef\@journalfull{Infrastructures}\gdef\@journalshort{Infrastructures}\gdef\@doiabbr{infrastructures}\gdef\@ISSN{2412-3811}}
\DeclareOption{inorganics}{\gdef\@journal{inorganics}\gdef\@journalfull{Inorganics}\gdef\@journalshort{Inorganics}\gdef\@doiabbr{inorganics}\gdef\@ISSN{2304-6740}}
\DeclareOption{insects}{\gdef\@journal{insects}\gdef\@journalfull{Insects}\gdef\@journalshort{Insects}\gdef\@doiabbr{insects}\gdef\@ISSN{2075-4450}}
\DeclareOption{instruments}{\gdef\@journal{instruments}\gdef\@journalfull{Instruments}\gdef\@journalshort{Instruments}\gdef\@doiabbr{instruments}\gdef\@ISSN{2410-390X}}
\DeclareOption{inventions}{\gdef\@journal{inventions}\gdef\@journalfull{Inventions}\gdef\@journalshort{Inventions}\gdef\@doiabbr{inventions}\gdef\@ISSN{2411-5134}}
\DeclareOption{iot}{\gdef\@journal{iot}\gdef\@journalfull{IoT}\gdef\@journalshort{IoT}\gdef\@doiabbr{iot}\gdef\@ISSN{2624-831X}\gdef\@continuouspages{yes}}
\DeclareOption{j}{\gdef\@journal{j}\gdef\@journalfull{J}\gdef\@journalshort{J}\gdef\@doiabbr{j}\gdef\@ISSN{2571-8800}\gdef\@continuouspages{yes}}
\DeclareOption{jal}{\gdef\@journal{jal}\gdef\@journalfull{Journal of Ageing and Longevity}\gdef\@journalshort{J. Ageing Longev.}\gdef\@doiabbr{jal}\gdef\@ISSN{2673-9259}\gdef\@continuouspages{yes}}
\DeclareOption{jcdd}{\gdef\@journal{jcdd}\gdef\@journalfull{Journal of Cardiovascular Development and Disease}\gdef\@journalshort{J. Cardiovasc. Dev. Dis.}\gdef\@doiabbr{jcdd}\gdef\@ISSN{2308-3425}}
\DeclareOption{jcm}{\gdef\@journal{jcm}\gdef\@journalfull{Journal of Clinical Medicine}\gdef\@journalshort{J. Clin. Med.}\gdef\@doiabbr{jcm}\gdef\@ISSN{2077-0383}}
\DeclareOption{jcp}{\gdef\@journal{jcp}\gdef\@journalfull{Journal of Cybersecurity and Privacy}\gdef\@journalshort{J. Cybersecur. Priv.}\gdef\@doiabbr{jcp}\gdef\@ISSN{2624-800X}\gdef\@continuouspages{yes}}
\DeclareOption{jcs}{\gdef\@journal{jcs}\gdef\@journalfull{Journal of Composites Science}\gdef\@journalshort{J. Compos. Sci.}\gdef\@doiabbr{jcs}\gdef\@ISSN{2504-477X}}
\DeclareOption{jcto}{\gdef\@journal{jcto}\gdef\@journalfull{Journal of Clinical \& Translational Ophthalmology}\gdef\@journalshort{J. Clin. Transl. Ophthalmol.}\gdef\@doiabbr{jcto}\gdef\@ISSN{2813-1053}\gdef\@continuouspages{yes}}
\DeclareOption{jdb}{\gdef\@journal{jdb}\gdef\@journalfull{Journal of Developmental Biology}\gdef\@journalshort{J. Dev. Biol.}\gdef\@doiabbr{jdb}\gdef\@ISSN{2221-3759}}
\DeclareOption{jeta}{\gdef\@journal{jeta}\gdef\@journalfull{Journal of Experimental and Theoretical Analyses}\gdef\@journalshort{J. Exp. Theor. Anal.}\gdef\@doiabbr{jeta}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{jfb}{\gdef\@journal{jfb}\gdef\@journalfull{Journal of Functional Biomaterials}\gdef\@journalshort{J. Funct. Biomater.}\gdef\@doiabbr{jfb}\gdef\@ISSN{2079-4983}}
\DeclareOption{jfmk}{\gdef\@journal{jfmk}\gdef\@journalfull{Journal of Functional Morphology and Kinesiology}\gdef\@journalshort{J. Funct. Morphol. Kinesiol.}\gdef\@doiabbr{jfmk}\gdef\@ISSN{2411-5142}}
\DeclareOption{jimaging}{\gdef\@journal{jimaging}\gdef\@journalfull{Journal of Imaging}\gdef\@journalshort{J. Imaging}\gdef\@doiabbr{jimaging}\gdef\@ISSN{2313-433X}}
\DeclareOption{jintelligence}{\gdef\@journal{jintelligence}\gdef\@journalfull{Journal of Intelligence}\gdef\@journalshort{J. Intell.}\gdef\@doiabbr{jintelligence}\gdef\@ISSN{2079-3200}}
\DeclareOption{jlpea}{\gdef\@journal{jlpea}\gdef\@journalfull{Journal of Low Power Electronics and Applications}\gdef\@journalshort{J. Low Power Electron. Appl.}\gdef\@doiabbr{jlpea}\gdef\@ISSN{2079-9268}}
\DeclareOption{jmmp}{\gdef\@journal{jmmp}\gdef\@journalfull{Journal of Manufacturing and Materials Processing}\gdef\@journalshort{J. Manuf. Mater. Process.}\gdef\@doiabbr{jmmp}\gdef\@ISSN{2504-4494}}
\DeclareOption{jmp}{\gdef\@journal{jmp}\gdef\@journalfull{Journal of Molecular Pathology}\gdef\@journalshort{J. Mol. Pathol.}\gdef\@doiabbr{jmp}\gdef\@ISSN{2673-5261}\gdef\@continuouspages{yes}}
\DeclareOption{jmse}{\gdef\@journal{jmse}\gdef\@journalfull{Journal of Marine Science and Engineering}\gdef\@journalshort{J. Mar. Sci. Eng.}\gdef\@doiabbr{jmse}\gdef\@ISSN{2077-1312}}
\DeclareOption{jne}{\gdef\@journal{jne}\gdef\@journalfull{Journal of Nuclear Engineering}\gdef\@journalshort{J. Nucl. Eng.}\gdef\@doiabbr{jne}\gdef\@ISSN{2673-4362}\gdef\@continuouspages{yes}}
\DeclareOption{jnt}{\gdef\@journal{jnt}\gdef\@journalfull{Journal of Nanotheranostics}\gdef\@journalshort{J. Nanotheranostics}\gdef\@doiabbr{jnt}\gdef\@ISSN{2624-845X}\gdef\@continuouspages{yes}}
\DeclareOption{jof}{\gdef\@journal{jof}\gdef\@journalfull{Journal of Fungi}\gdef\@journalshort{J. Fungi}\gdef\@doiabbr{jof}\gdef\@ISSN{2309-608X}}
\DeclareOption{joitmc}{\gdef\@journal{joitmc}\gdef\@journalfull{Journal of Open Innovation: Technology, Market, and Complexity}\gdef\@journalshort{J. Open Innov. Technol. Mark. Complex.}\gdef\@doiabbr{joitmc}\gdef\@ISSN{2199-8531}}
\DeclareOption{jor}{\gdef\@journal{jor}\gdef\@journalfull{Journal of Respiration}\gdef\@journalshort{J. Respir.}\gdef\@doiabbr{jor}\gdef\@ISSN{2673-527X}\gdef\@continuouspages{yes}}
\DeclareOption{journalmedia}{\gdef\@journal{journalmedia}\gdef\@journalfull{Journalism and Media}\gdef\@journalshort{Journal. Media}\gdef\@doiabbr{journalmedia}\gdef\@ISSN{2673-5172}\gdef\@continuouspages{yes}}
\DeclareOption{jox}{\gdef\@journal{jox}\gdef\@journalfull{Journal of Xenobiotics}\gdef\@journalshort{J. Xenobiot.}\gdef\@doiabbr{jox}\gdef\@ISSN{2039-4713}\gdef\@continuouspages{yes}}
\DeclareOption{jpm}{\gdef\@journal{jpm}\gdef\@journalfull{Journal of Personalized Medicine}\gdef\@journalshort{J. Pers. Med.}\gdef\@doiabbr{jpm}\gdef\@ISSN{2075-4426}}
\DeclareOption{jrfm}{\gdef\@journal{jrfm}\gdef\@journalfull{Journal of Risk and Financial Management}\gdef\@journalshort{J. Risk Financial Manag.}\gdef\@doiabbr{jrfm}\gdef\@ISSN{1911-8074}}
\DeclareOption{jsan}{\gdef\@journal{jsan}\gdef\@journalfull{Journal of Sensor and Actuator Networks}\gdef\@journalshort{J. Sens. Actuator Netw.}\gdef\@doiabbr{jsan}\gdef\@ISSN{2224-2708}}
\DeclareOption{jtaer}{\gdef\@journal{jtaer}\gdef\@journalfull{Journal of Theoretical and Applied Electronic Commerce Research}\gdef\@journalshort{J. Theor. Appl. Electron. Commer. Res.}\gdef\@doiabbr{jtaer}\gdef\@ISSN{0718-1876}\gdef\@continuouspages{yes}}
\DeclareOption{jvd}{\gdef\@journal{jvd}\gdef\@journalfull{Journal of Vascular Diseases}\gdef\@journalshort{JVD}\gdef\@doiabbr{jvd}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{jzbg}{\gdef\@journal{jzbg}\gdef\@journalfull{Journal of Zoological and Botanical Gardens}\gdef\@journalshort{J. Zool. Bot. Gard.}\gdef\@doiabbr{jzbg}\gdef\@ISSN{2673-5636}\gdef\@continuouspages{yes}}
%\DeclareOption{kidney}{\gdef\@journal{kidney}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{kidneydial}{\gdef\@journal{kidneydial}\gdef\@journalfull{Kidney and Dialysis}\gdef\@journalshort{Kidney Dial.}\gdef\@doiabbr{kinasesphosphatases}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{kinasesphosphatases}{\gdef\@journal{kinasesphosphatases}\gdef\@journalfull{Kinases and Phosphatases}\gdef\@journalshort{Kinases Phosphatases}\gdef\@doiabbr{kinasesphosphatases}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{knowledge}{\gdef\@journal{knowledge}\gdef\@journalfull{Knowledge}\gdef\@journalshort{Knowledge}\gdef\@doiabbr{knowledge}\gdef\@ISSN{2673-9585}\gdef\@continuouspages{yes}}
\DeclareOption{land}{\gdef\@journal{land}\gdef\@journalfull{Land}\gdef\@journalshort{Land}\gdef\@doiabbr{land}\gdef\@ISSN{2073-445X}}
\DeclareOption{languages}{\gdef\@journal{languages}\gdef\@journalfull{Languages}\gdef\@journalshort{Languages}\gdef\@doiabbr{languages}\gdef\@ISSN{2226-471X}}
\DeclareOption{laws}{\gdef\@journal{laws}\gdef\@journalfull{Laws}\gdef\@journalshort{Laws}\gdef\@doiabbr{laws}\gdef\@ISSN{2075-471X}}
\DeclareOption{life}{\gdef\@journal{life}\gdef\@journalfull{Life}\gdef\@journalshort{Life}\gdef\@doiabbr{life}\gdef\@ISSN{2075-1729}}
\DeclareOption{limnolrev}{\gdef\@journal{limnolrev}\gdef\@journalfull{Limnological Review}\gdef\@journalshort{Limnol. Rev.}\gdef\@doiabbr{limnolrev}\gdef\@ISSN{2300-7575}\gdef\@continuouspages{yes}}
\DeclareOption{lipidology}{\gdef\@journal{lipidology}\gdef\@journalfull{Lipidology}\gdef\@journalshort{Lipidology}\gdef\@doiabbr{lipidology}\gdef\@ISSN{2813-7086}\gdef\@continuouspages{yes}}
\DeclareOption{liquids}{\gdef\@journal{liquids}\gdef\@journalfull{Liquids}\gdef\@journalshort{Liquids}\gdef\@doiabbr{liquids}\gdef\@ISSN{2673-8015}\gdef\@continuouspages{yes}}
\DeclareOption{literature}{\gdef\@journal{literature}\gdef\@journalfull{Literature}\gdef\@journalshort{Literature}\gdef\@doiabbr{literature}\gdef\@ISSN{2410-9789}\gdef\@continuouspages{yes}}
\DeclareOption{livers}{\gdef\@journal{livers}\gdef\@journalfull{Livers}\gdef\@journalshort{Livers}\gdef\@doiabbr{livers}\gdef\@ISSN{2673-4389}\gdef\@continuouspages{yes}}
\DeclareOption{logics}{\gdef\@journal{logics}\gdef\@journalfull{Logics}\gdef\@journalshort{Logics}\gdef\@doiabbr{logics}\gdef\@ISSN{2813-0405}\gdef\@continuouspages{yes}}
\DeclareOption{logistics}{\gdef\@journal{logistics}\gdef\@journalfull{Logistics}\gdef\@journalshort{Logistics}\gdef\@doiabbr{logistics}\gdef\@ISSN{2305-6290}}
\DeclareOption{lubricants}{\gdef\@journal{lubricants}\gdef\@journalfull{Lubricants}\gdef\@journalshort{Lubricants}\gdef\@doiabbr{lubricants}\gdef\@ISSN{2075-4442}}
\DeclareOption{lymphatics}{\gdef\@journal{lymphatics}\gdef\@journalfull{Lymphatics}\gdef\@journalshort{Lymphatics}\gdef\@doiabbr{lymphatics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}	
\DeclareOption{machines}{\gdef\@journal{machines}\gdef\@journalfull{Machines}\gdef\@journalshort{Machines}\gdef\@doiabbr{machines}\gdef\@ISSN{2075-1702}}
\DeclareOption{macromol}{\gdef\@journal{macromol}\gdef\@journalfull{Macromol}\gdef\@journalshort{Macromol}\gdef\@doiabbr{macromol}\gdef\@ISSN{2673-6209}\gdef\@continuouspages{yes}}
\DeclareOption{magnetism}{\gdef\@journal{magnetism}\gdef\@journalfull{Magnetism}\gdef\@journalshort{Magnetism}\gdef\@doiabbr{magnetism}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{magnetochemistry}{\gdef\@journal{magnetochemistry}\gdef\@journalfull{Magnetochemistry}\gdef\@journalshort{Magnetochemistry}\gdef\@doiabbr{magnetochemistry}\gdef\@ISSN{2312-7481}}
\DeclareOption{make}{\gdef\@journal{make}\gdef\@journalfull{Machine Learning and Knowledge Extraction}\gdef\@journalshort{Mach. Learn. Knowl. Extr.}\gdef\@doiabbr{make}\gdef\@ISSN{2504-4990}\gdef\@continuouspages{yes}}
\DeclareOption{marinedrugs}{\gdef\@journal{marinedrugs}\gdef\@journalfull{Marine Drugs}\gdef\@journalshort{Mar. Drugs}\gdef\@doiabbr{md}\gdef\@ISSN{1660-3397}}
\DeclareOption{materials}{\gdef\@journal{materials}\gdef\@journalfull{Materials}\gdef\@journalshort{Materials}\gdef\@doiabbr{ma}\gdef\@ISSN{1996-1944}}
\DeclareOption{materproc}{\gdef\@journal{materproc}\gdef\@journalfull{Materials Proceedings}\gdef\@journalshort{Mater. Proc.}\gdef\@doiabbr{materproc}\gdef\@ISSN{2673-4605}}
\DeclareOption{mathematics}{\gdef\@journal{mathematics}\gdef\@journalfull{Mathematics}\gdef\@journalshort{Mathematics}\gdef\@doiabbr{math}\gdef\@ISSN{2227-7390}}
\DeclareOption{mca}{\gdef\@journal{mca}\gdef\@journalfull{Mathematical and Computational Applications}\gdef\@journalshort{Math. Comput. Appl.}\gdef\@doiabbr{mca}\gdef\@ISSN{2297-8747}}
\DeclareOption{measurements}{\gdef\@journal{measurements}\gdef\@journalfull{Measurements}\gdef\@journalshort{Measurements}\gdef\@doiabbr{measurements}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{medicina}{\gdef\@journal{medicina}\gdef\@journalfull{Medicina}\gdef\@journalshort{Medicina}\gdef\@doiabbr{medicina}\gdef\@ISSN{1648-9144}}
\DeclareOption{medicines}{\gdef\@journal{medicines}\gdef\@journalfull{Medicines}\gdef\@journalshort{Medicines}\gdef\@doiabbr{medicines}\gdef\@ISSN{2305-6320}}
\DeclareOption{medsci}{\gdef\@journal{medsci}\gdef\@journalfull{Medical Sciences}\gdef\@journalshort{Med. Sci.}\gdef\@doiabbr{medsci}\gdef\@ISSN{2076-3271}}
\DeclareOption{membranes}{\gdef\@journal{membranes}\gdef\@journalfull{Membranes}\gdef\@journalshort{Membranes}\gdef\@doiabbr{membranes}\gdef\@ISSN{2077-0375}}
\DeclareOption{merits}{\gdef\@journal{merits}\gdef\@journalfull{Merits}\gdef\@journalshort{Merits}\gdef\@doiabbr{merits}\gdef\@ISSN{2673-8104}\gdef\@continuouspages{yes}}
\DeclareOption{metabolites}{\gdef\@journal{metabolites}\gdef\@journalfull{Metabolites}\gdef\@journalshort{Metabolites}\gdef\@doiabbr{metabo}\gdef\@ISSN{2218-1989}}
\DeclareOption{metals}{\gdef\@journal{metals}\gdef\@journalfull{Metals}\gdef\@journalshort{Metals}\gdef\@doiabbr{met}\gdef\@ISSN{2075-4701}}
\DeclareOption{meteorology}{\gdef\@journal{meteorology}\gdef\@journalfull{Meteorology}\gdef\@journalshort{Meteorology}\gdef\@doiabbr{meteorology}\gdef\@ISSN{2674-0494}\gdef\@continuouspages{yes}}
\DeclareOption{methane}{\gdef\@journal{methane}\gdef\@journalfull{Methane}\gdef\@journalshort{Methane}\gdef\@doiabbr{methane}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{metrology}{\gdef\@journal{metrology}\gdef\@journalfull{Metrology}\gdef\@journalshort{Metrology}\gdef\@doiabbr{metrology}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{micro}{\gdef\@journal{micro}\gdef\@journalfull{Micro}\gdef\@journalshort{Micro}\gdef\@doiabbr{micro}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{microarrays}{\gdef\@journal{microarrays}\gdef\@journalfull{Microarrays}\gdef\@journalshort{Microarrays}\gdef\@doiabbr{microarrays}\gdef\@ISSN{2076-3905}}
\DeclareOption{microbiolres}{\gdef\@journal{microbiolres}\gdef\@journalfull{Microbiology Research}\gdef\@journalshort{Microbiol. Res.}\gdef\@doiabbr{microbiolres}\gdef\@ISSN{2036-7481}\gdef\@continuouspages{yes}}
\DeclareOption{micromachines}{\gdef\@journal{micromachines}\gdef\@journalfull{Micromachines}\gdef\@journalshort{Micromachines}\gdef\@doiabbr{mi}\gdef\@ISSN{2072-666X}}
\DeclareOption{microorganisms}{\gdef\@journal{microorganisms}\gdef\@journalfull{Microorganisms}\gdef\@journalshort{Microorganisms}\gdef\@doiabbr{microorganisms}\gdef\@ISSN{2076-2607}}
\DeclareOption{microplastics}{\gdef\@journal{microplastics}\gdef\@journalfull{Microplastics}\gdef\@journalshort{Microplastics}\gdef\@doiabbr{microplastics}\gdef\@ISSN{2673-8929}\gdef\@continuouspages{yes}}
\DeclareOption{minerals}{\gdef\@journal{minerals}\gdef\@journalfull{Minerals}\gdef\@journalshort{Minerals}\gdef\@doiabbr{min}\gdef\@ISSN{2075-163X}}
\DeclareOption{mining}{\gdef\@journal{mining}\gdef\@journalfull{Mining}\gdef\@journalshort{Mining}\gdef\@doiabbr{mining}\gdef\@ISSN{2673-6489}\gdef\@continuouspages{yes}}
\DeclareOption{modelling}{\gdef\@journal{modelling}\gdef\@journalfull{Modelling}\gdef\@journalshort{Modelling}\gdef\@doiabbr{modelling}\gdef\@ISSN{2673-3951}\gdef\@continuouspages{yes}}
\DeclareOption{molbank}{\gdef\@journal{molbank}\gdef\@journalfull{Molbank}\gdef\@journalshort{Molbank}\gdef\@doiabbr{M}\gdef\@ISSN{1422-8599}}
\DeclareOption{molecules}{\gdef\@journal{molecules}\gdef\@journalfull{Molecules}\gdef\@journalshort{Molecules}\gdef\@doiabbr{molecules}\gdef\@ISSN{1420-3049}}
\DeclareOption{mps}{\gdef\@journal{mps}\gdef\@journalfull{Methods and Protocols}\gdef\@journalshort{Methods Protoc.}\gdef\@doiabbr{mps}\gdef\@ISSN{2409-9279}}
\DeclareOption{msf}{\gdef\@journal{msf}\gdef\@journalfull{Medical Sciences Forum}\gdef\@journalshort{Med. Sci. Forum}\gdef\@doiabbr{msf}\gdef\@ISSN{2673-9992}}
\DeclareOption{mti}{\gdef\@journal{mti}\gdef\@journalfull{Multimodal Technologies and Interaction}\gdef\@journalshort{Multimodal Technol. Interact.}\gdef\@doiabbr{mti}\gdef\@ISSN{2414-4088}}
\DeclareOption{muscles}{\gdef\@journal{muscles}\gdef\@journalfull{Muscles}\gdef\@journalshort{Muscles}\gdef\@doiabbr{muscles}\gdef\@ISSN{2813-0413}\gdef\@continuouspages{yes}}
\DeclareOption{nanoenergyadv}{\gdef\@journal{nanoenergyadv}\gdef\@journalfull{Nanoenergy Advances}\gdef\@journalshort{Nanoenergy Adv.}\gdef\@doiabbr{nanoenergyadv}\gdef\@ISSN{2673-706X}\gdef\@continuouspages{yes}}
\DeclareOption{nanomanufacturing}{\gdef\@journal{nanomanufacturing}\gdef\@journalfull{Nanomanufacturing}\gdef\@journalshort{Nanomanufacturing}\gdef\@doiabbr{nanomanufacturing}\gdef\@ISSN{2673-687X}\gdef\@continuouspages{yes}}
\DeclareOption{nanomaterials}{\gdef\@journal{nanomaterials}\gdef\@journalfull{Nanomaterials}\gdef\@journalshort{Nanomaterials}\gdef\@doiabbr{nano}\gdef\@ISSN{2079-4991}}
\DeclareOption{ncrna}{\gdef\@journal{ncrna}\gdef\@journalfull{Non-Coding RNA}\gdef\@journalshort{Non-Coding RNA}\gdef\@doiabbr{ncrna}\gdef\@ISSN{2311-553X}}
\DeclareOption{ndt}{\gdef\@journal{ndt}\gdef\@journalfull{NDT}\gdef\@journalshort{NDT}\gdef\@doiabbr{ndt}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{network}{\gdef\@journal{network}\gdef\@journalfull{Network}\gdef\@journalshort{Network}\gdef\@doiabbr{network}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{neuroglia}{\gdef\@journal{neuroglia}\gdef\@journalfull{Neuroglia}\gdef\@journalshort{Neuroglia}\gdef\@doiabbr{neuroglia}\gdef\@ISSN{2571-6980}\gdef\@continuouspages{yes}}
\DeclareOption{neurolint}{\gdef\@journal{neurolint}\gdef\@journalfull{Neurology International}\gdef\@journalshort{Neurol. Int.}\gdef\@doiabbr{neurolint}\gdef\@ISSN{2035-8377}\gdef\@continuouspages{yes}}
\DeclareOption{neurosci}{\gdef\@journal{neurosci}\gdef\@journalfull{NeuroSci}\gdef\@journalshort{NeuroSci}\gdef\@doiabbr{neurosci}\gdef\@ISSN{2673-4087}\gdef\@continuouspages{yes}}
\DeclareOption{nitrogen}{\gdef\@journal{nitrogen}\gdef\@journalfull{Nitrogen}\gdef\@journalshort{Nitrogen}\gdef\@doiabbr{nitrogen}\gdef\@ISSN{2504-3129}\gdef\@continuouspages{yes}}
\DeclareOption{notspecified}{\gdef\@journal{notspecified}\gdef\@journalfull{Journal Not Specified}\gdef\@journalshort{Journal Not Specified}\gdef\@doiabbr{}\gdef\@ISSN{}}
%%\DeclareOption{nri}{\gdef\@journal{nri}\gdef\@journalfull{Natural Resources Informatics}\gdef\@journalshort{Nat. Resour. Inform.}\gdef\@doiabbr{nri}\gdef\@ISSN{2673-981X}\gdef\@continuouspages{yes}}
\DeclareOption{nursrep}{\gdef\@journal{nursrep}\gdef\@journalfull{Nursing Reports}\gdef\@journalshort{Nurs. Rep.}\gdef\@doiabbr{nursrep}\gdef\@ISSN{2039-4403}\gdef\@continuouspages{yes}}
\DeclareOption{nutraceuticals}{\gdef\@journal{nutraceuticals}\gdef\@journalfull{Nutraceuticals}\gdef\@journalshort{Nutraceuticals}\gdef\@doiabbr{nutraceuticals}\gdef\@ISSN{1661-3821}\gdef\@continuouspages{yes}}
\DeclareOption{nutrients}{\gdef\@journal{nutrients}\gdef\@journalfull{Nutrients}\gdef\@journalshort{Nutrients}\gdef\@doiabbr{nu}\gdef\@ISSN{2072-6643}}
\DeclareOption{obesities}{\gdef\@journal{obesities}\gdef\@journalfull{Obesities}\gdef\@journalshort{Obesities}\gdef\@doiabbr{obesities}\gdef\@ISSN{2673-4168}\gdef\@continuouspages{yes}}
\DeclareOption{oceans}{\gdef\@journal{oceans}\gdef\@journalfull{Oceans}\gdef\@journalshort{Oceans}\gdef\@doiabbr{oceans}\gdef\@ISSN{2673-1924}\gdef\@continuouspages{yes}}
\DeclareOption{ohbm}{\gdef\@journal{ohbm}\gdef\@journalfull{Journal of Otorhinolaryngology, Hearing and Balance Medicine}\gdef\@journalshort{J. Otorhinolaryngol. Hear. Balance Med.}\gdef\@doiabbr{ohbm}\gdef\@ISSN{2504-463X}}
\DeclareOption{onco}{\gdef\@journal{onco}\gdef\@journalfull{Onco}\gdef\@journalshort{Onco}\gdef\@doiabbr{onco}\gdef\@ISSN{2673-7523}\gdef\@continuouspages{yes}}
%\DeclareOption{oncopathology}{\gdef\@journal{oncopathology}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{optics}{\gdef\@journal{optics}\gdef\@journalfull{Optics}\gdef\@journalshort{Optics}\gdef\@doiabbr{opt}\gdef\@ISSN{2673-3269}\gdef\@continuouspages{yes}}
\DeclareOption{oral}{\gdef\@journal{oral}\gdef\@journalfull{Oral}\gdef\@journalshort{Oral}\gdef\@doiabbr{oral}\gdef\@ISSN{2673-6373}\gdef\@continuouspages{yes}}
\DeclareOption{organics}{\gdef\@journal{organics}\gdef\@journalfull{Organics}\gdef\@journalshort{Organics}\gdef\@doiabbr{org}\gdef\@ISSN{2673-401X}\gdef\@continuouspages{yes}}
\DeclareOption{organoids}{\gdef\@journal{organoids}\gdef\@journalfull{Organoids}\gdef\@journalshort{Organoids}\gdef\@doiabbr{organoids}\gdef\@ISSN{2674-1172}\gdef\@continuouspages{yes}}
\DeclareOption{osteology}{\gdef\@journal{osteology}\gdef\@journalfull{Osteology}\gdef\@journalshort{Osteology}\gdef\@doiabbr{osteology}\gdef\@ISSN{2673-4036}\gdef\@continuouspages{yes}}
\DeclareOption{oxygen}{\gdef\@journal{oxygen}\gdef\@journalfull{Oxygen}\gdef\@journalshort{Oxygen}\gdef\@doiabbr{oxygen}\gdef\@ISSN{2673-9801}\gdef\@continuouspages{yes}}
\DeclareOption{parasites}{\gdef\@journal{parasites}\gdef\@journalfull{Parasites}\gdef\@journalshort{Parasites}\gdef\@doiabbr{parasites}\gdef\@ISSN{2673-5946}}
\DeclareOption{parasitologia}{\gdef\@journal{parasitologia}\gdef\@journalfull{Parasitologia}\gdef\@journalshort{Parasitologia}\gdef\@doiabbr{parasitologia}\gdef\@ISSN{2673-6772}\gdef\@continuouspages{yes}}
\DeclareOption{particles}{\gdef\@journal{particles}\gdef\@journalfull{Particles}\gdef\@journalshort{Particles}\gdef\@doiabbr{particles}\gdef\@ISSN{2571-712X}\gdef\@continuouspages{yes}}
\DeclareOption{pathogens}{\gdef\@journal{pathogens}\gdef\@journalfull{Pathogens}\gdef\@journalshort{Pathogens}\gdef\@doiabbr{pathogens}\gdef\@ISSN{2076-0817}}
\DeclareOption{pathophysiology}{\gdef\@journal{pathophysiology}\gdef\@journalfull{Pathophysiology}\gdef\@journalshort{Pathophysiology}\gdef\@doiabbr{pathophysiology}\gdef\@ISSN{0928-4680}\gdef\@continuouspages{yes}}
\DeclareOption{pediatrrep}{\gdef\@journal{pediatrrep}\gdef\@journalfull{Pediatric Reports}\gdef\@journalshort{Pediatr. Rep.}\gdef\@doiabbr{pediatric}\gdef\@ISSN{2036-7503}\gdef\@continuouspages{yes}}
\DeclareOption{pets}{\gdef\@journal{pets}\gdef\@journalfull{Pets}\gdef\@journalshort{Pets}\gdef\@doiabbr{pets}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{pharmaceuticals}{\gdef\@journal{pharmaceuticals}\gdef\@journalfull{Pharmaceuticals}\gdef\@journalshort{Pharmaceuticals}\gdef\@doiabbr{ph}\gdef\@ISSN{1424-8247}}
\DeclareOption{pharmaceutics}{\gdef\@journal{pharmaceutics}\gdef\@journalfull{Pharmaceutics}\gdef\@journalshort{Pharmaceutics}\gdef\@doiabbr{pharmaceutics}\gdef\@ISSN{1999-4923}}
\DeclareOption{pharmacoepidemiology}{\gdef\@journal{pharmacoepidemiology}\gdef\@journalfull{Pharmacoepidemiology}\gdef\@journalshort{Pharmacoepidemiology}\gdef\@doiabbr{pharma}\gdef\@ISSN{2813-0618}\gdef\@continuouspages{yes}}
\DeclareOption{pharmacy}{\gdef\@journal{pharmacy}\gdef\@journalfull{Pharmacy}\gdef\@journalshort{Pharmacy}\gdef\@doiabbr{pharmacy}\gdef\@ISSN{2226-4787}}
\DeclareOption{philosophies}{\gdef\@journal{philosophies}\gdef\@journalfull{Philosophies}\gdef\@journalshort{Philosophies}\gdef\@doiabbr{philosophies}\gdef\@ISSN{2409-9287}}
\DeclareOption{photochem}{\gdef\@journal{photochem}\gdef\@journalfull{Photochem}\gdef\@journalshort{Photochem}\gdef\@doiabbr{photochem}\gdef\@ISSN{2673-7256}\gdef\@continuouspages{yes}}
\DeclareOption{photonics}{\gdef\@journal{photonics}\gdef\@journalfull{Photonics}\gdef\@journalshort{Photonics}\gdef\@doiabbr{photonics}\gdef\@ISSN{2304-6732}}
\DeclareOption{phycology}{\gdef\@journal{phycology}\gdef\@journalfull{Phycology}\gdef\@journalshort{Phycology}\gdef\@doiabbr{phycology}\gdef\@ISSN{2673-9410}\gdef\@continuouspages{yes}}
\DeclareOption{physchem}{\gdef\@journal{physchem}\gdef\@journalfull{Physchem}\gdef\@journalshort{Physchem}\gdef\@doiabbr{physchem}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{physics}{\gdef\@journal{physics}\gdef\@journalfull{Physics}\gdef\@journalshort{Physics}\gdef\@doiabbr{physics}\gdef\@ISSN{2624-8174}\gdef\@continuouspages{yes}}
\DeclareOption{physiologia}{\gdef\@journal{physiologia}\gdef\@journalfull{Physiologia}\gdef\@journalshort{Physiologia}\gdef\@doiabbr{physiologia}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{plants}{\gdef\@journal{plants}\gdef\@journalfull{Plants}\gdef\@journalshort{Plants}\gdef\@doiabbr{plants}\gdef\@ISSN{2223-7747}}
\DeclareOption{plasma}{\gdef\@journal{plasma}\gdef\@journalfull{Plasma}\gdef\@journalshort{Plasma}\gdef\@doiabbr{plasma}\gdef\@ISSN{2571-6182}\gdef\@continuouspages{yes}}
\DeclareOption{platforms}{\gdef\@journal{platforms}\gdef\@journalfull{Platforms}\gdef\@journalshort{Platforms}\gdef\@doiabbr{platforms}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{pollutants}{\gdef\@journal{pollutants}\gdef\@journalfull{Pollutants}\gdef\@journalshort{Pollutants}\gdef\@doiabbr{pollutants}\gdef\@ISSN{2673-4672}\gdef\@continuouspages{yes}}
\DeclareOption{polymers}{\gdef\@journal{polymers}\gdef\@journalfull{Polymers}\gdef\@journalshort{Polymers}\gdef\@doiabbr{polym}\gdef\@ISSN{2073-4360}}
\DeclareOption{polysaccharides}{\gdef\@journal{polysaccharides}\gdef\@journalfull{Polysaccharides}\gdef\@journalshort{Polysaccharides}\gdef\@doiabbr{polysaccharides}\gdef\@ISSN{2673-4176}\gdef\@continuouspages{yes}}
\DeclareOption{poultry}{\gdef\@journal{poultry}\gdef\@journalfull{Poultry}\gdef\@journalshort{Poultry}\gdef\@doiabbr{poultry}\gdef\@ISSN{2674-1164}\gdef\@continuouspages{yes}}
\DeclareOption{powders}{\gdef\@journal{powders}\gdef\@journalfull{Powders}\gdef\@journalshort{Powders}\gdef\@doiabbr{powders}\gdef\@ISSN{2674-0516}\gdef\@continuouspages{yes}}
\DeclareOption{preprints}{\gdef\@journal{preprints}\gdef\@journalfull{Preprints}\gdef\@journalshort{Preprints}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{proceedings}{\gdef\@journal{proceedings}\gdef\@journalfull{Proceedings}\gdef\@journalshort{Proceedings}\gdef\@doiabbr{proceedings}\gdef\@ISSN{2504-3900}}
\DeclareOption{processes}{\gdef\@journal{processes}\gdef\@journalfull{Processes}\gdef\@journalshort{Processes}\gdef\@doiabbr{pr}\gdef\@ISSN{2227-9717}}
\DeclareOption{prosthesis}{\gdef\@journal{prosthesis}\gdef\@journalfull{Prosthesis}\gdef\@journalshort{Prosthesis}\gdef\@doiabbr{prosthesis}\gdef\@ISSN{2673-1592}\gdef\@continuouspages{yes}}
\DeclareOption{proteomes}{\gdef\@journal{proteomes}\gdef\@journalfull{Proteomes}\gdef\@journalshort{Proteomes}\gdef\@doiabbr{proteomes}\gdef\@ISSN{2227-7382}}
\DeclareOption{psf}{\gdef\@journal{psf}\gdef\@journalfull{Physical Sciences Forum}\gdef\@journalshort{Phys. Sci. Forum}\gdef\@doiabbr{psf}\gdef\@ISSN{2673-9984}}
\DeclareOption{psych}{\gdef\@journal{psych}\gdef\@journalfull{Psych}\gdef\@journalshort{Psych}\gdef\@doiabbr{psych}\gdef\@ISSN{2624-8611}\gdef\@continuouspages{yes}}
\DeclareOption{psychiatryint}{\gdef\@journal{psychiatryint}\gdef\@journalfull{Psychiatry International}\gdef\@journalshort{Psychiatry Int.}\gdef\@doiabbr{psychiatryint}\gdef\@ISSN{2673-5318}\gdef\@continuouspages{yes}}
\DeclareOption{psychoactives}{\gdef\@journal{psychoactives}\gdef\@journalfull{Psychoactives}\gdef\@journalshort{Psychoactives}\gdef\@doiabbr{psychoactives}\gdef\@ISSN{2813-1851}\gdef\@continuouspages{yes}}
\DeclareOption{publications}{\gdef\@journal{publications}\gdef\@journalfull{Publications}\gdef\@journalshort{Publications}\gdef\@doiabbr{publications}\gdef\@ISSN{2304-6775}}
\DeclareOption{quantumrep}{\gdef\@journal{quantumrep}\gdef\@journalfull{Quantum Reports}\gdef\@journalshort{Quantum Rep.}\gdef\@doiabbr{quantum}\gdef\@ISSN{2624-960X}\gdef\@continuouspages{yes}}
\DeclareOption{quaternary}{\gdef\@journal{quaternary}\gdef\@journalfull{Quaternary}\gdef\@journalshort{Quaternary}\gdef\@doiabbr{quat}\gdef\@ISSN{2571-550X}}
\DeclareOption{qubs}{\gdef\@journal{qubs}\gdef\@journalfull{Quantum Beam Science}\gdef\@journalshort{Quantum Beam Sci.}\gdef\@doiabbr{qubs}\gdef\@ISSN{2412-382X}}
\DeclareOption{radiation}{\gdef\@journal{radiation}\gdef\@journalfull{Radiation}\gdef\@journalshort{Radiation}\gdef\@doiabbr{radiation}\gdef\@ISSN{2673-592X}\gdef\@continuouspages{yes}}
\DeclareOption{reactions}{\gdef\@journal{reactions}\gdef\@journalfull{Reactions}\gdef\@journalshort{Reactions}\gdef\@doiabbr{reactions}\gdef\@ISSN{2624-781X}\gdef\@continuouspages{yes}}
\DeclareOption{receptors}{\gdef\@journal{receptors}\gdef\@journalfull{Receptors}\gdef\@journalshort{Receptors}\gdef\@doiabbr{receptors}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{recycling}{\gdef\@journal{recycling}\gdef\@journalfull{Recycling}\gdef\@journalshort{Recycling}\gdef\@doiabbr{recycling}\gdef\@ISSN{2313-4321}}
\DeclareOption{regeneration}{\gdef\@journal{regeneration}\gdef\@journalfull{Regeneration}\gdef\@journalshort{Regeneration}\gdef\@doiabbr{regeneration}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{religions}{\gdef\@journal{religions}\gdef\@journalfull{Religions}\gdef\@journalshort{Religions}\gdef\@doiabbr{rel}\gdef\@ISSN{2077-1444}}
\DeclareOption{remotesensing}{\gdef\@journal{remotesensing}\gdef\@journalfull{Remote Sensing}\gdef\@journalshort{Remote Sens.}\gdef\@doiabbr{rs}\gdef\@ISSN{2072-4292}}
\DeclareOption{reports}{\gdef\@journal{reports}\gdef\@journalfull{Reports}\gdef\@journalshort{Reports}\gdef\@doiabbr{reports}\gdef\@ISSN{2571-841X}}
\DeclareOption{reprodmed}{\gdef\@journal{reprodmed}\gdef\@journalfull{Reproductive Medicine}\gdef\@journalshort{Reprod. Med.}\gdef\@doiabbr{reprodmed}\gdef\@ISSN{2673-3897}\gdef\@continuouspages{yes}}
\DeclareOption{resources}{\gdef\@journal{resources}\gdef\@journalfull{Resources}\gdef\@journalshort{Resources}\gdef\@doiabbr{resources}\gdef\@ISSN{2079-9276}}
\DeclareOption{rheumato}{\gdef\@journal{rheumato}\gdef\@journalfull{Rheumato}\gdef\@journalshort{Rheumato}\gdef\@doiabbr{rheumato}\gdef\@ISSN{2674-0621}\gdef\@continuouspages{yes}}
\DeclareOption{risks}{\gdef\@journal{risks}\gdef\@journalfull{Risks}\gdef\@journalshort{Risks}\gdef\@doiabbr{risks}\gdef\@ISSN{2227-9091}}
\DeclareOption{robotics}{\gdef\@journal{robotics}\gdef\@journalfull{Robotics}\gdef\@journalshort{Robotics}\gdef\@doiabbr{robotics}\gdef\@ISSN{2218-6581}}
\DeclareOption{ruminants}{\gdef\@journal{ruminants}\gdef\@journalfull{Ruminants}\gdef\@journalshort{Ruminants}\gdef\@doiabbr{ruminants}\gdef\@ISSN{2673-933X}\gdef\@continuouspages{yes}}
\DeclareOption{safety}{\gdef\@journal{safety}\gdef\@journalfull{Safety}\gdef\@journalshort{Safety}\gdef\@doiabbr{safety}\gdef\@ISSN{2313-576X}}
\DeclareOption{sci}{\gdef\@journal{sci}\gdef\@journalfull{Sci}\gdef\@journalshort{Sci}\gdef\@doiabbr{sci}\gdef\@ISSN{2413-4155}}
\DeclareOption{scipharm}{\gdef\@journal{scipharm}\gdef\@journalfull{Scientia Pharmaceutica}\gdef\@journalshort{Sci. Pharm.}\gdef\@doiabbr{scipharm}\gdef\@ISSN{2218-0532}}
\DeclareOption{sclerosis}{\gdef\@journal{sclerosis}\gdef\@journalfull{Sclerosis}\gdef\@journalshort{Sclerosis}\gdef\@doiabbr{sclerosis}\gdef\@ISSN{2813-3064}\gdef\@continuouspages{yes}}
\DeclareOption{seeds}{\gdef\@journal{seeds}\gdef\@journalfull{Seeds}\gdef\@journalshort{Seeds}\gdef\@doiabbr{seeds}\gdef\@ISSN{2674-1024}\gdef\@continuouspages{yes}}
\DeclareOption{sensors}{\gdef\@journal{sensors}\gdef\@journalfull{Sensors}\gdef\@journalshort{Sensors}\gdef\@doiabbr{s}\gdef\@ISSN{1424-8220}}
\DeclareOption{separations}{\gdef\@journal{separations}\gdef\@journalfull{Separations}\gdef\@journalshort{Separations}\gdef\@doiabbr{separations}\gdef\@ISSN{2297-8739}}
\DeclareOption{sexes}{\gdef\@journal{sexes}\gdef\@journalfull{Sexes}\gdef\@journalshort{Sexes}\gdef\@doiabbr{sexes}\gdef\@ISSN{2411-5118}\gdef\@continuouspages{yes}}
\DeclareOption{signals}{\gdef\@journal{signals}\gdef\@journalfull{Signals}\gdef\@journalshort{Signals}\gdef\@doiabbr{signals}\gdef\@ISSN{2624-6120}\gdef\@continuouspages{yes}}
\DeclareOption{sinusitis}{\gdef\@journal{sinusitis}\gdef\@journalfull{Sinusitis}\gdef\@journalshort{Sinusitis}\gdef\@doiabbr{sinusitis}\gdef\@ISSN{2309-107X}\gdef\@continuouspages{yes}}
\DeclareOption{skins}{\gdef\@journal{skins}\gdef\@journalfull{Skins}\gdef\@journalshort{Skins}\gdef\@doiabbr{skins}\gdef\@ISSN{}}
\DeclareOption{smartcities}{\gdef\@journal{smartcities}\gdef\@journalfull{Smart Cities}\gdef\@journalshort{Smart Cities}\gdef\@doiabbr{smartcities}\gdef\@ISSN{2624-6511}\gdef\@continuouspages{yes}}
\DeclareOption{sna}{\gdef\@journal{sna}\gdef\@journalfull{Sinusitis and Asthma}\gdef\@journalshort{Sinusitis Asthma}\gdef\@doiabbr{sna}\gdef\@ISSN{2624-7003}}
\DeclareOption{societies}{\gdef\@journal{societies}\gdef\@journalfull{Societies}\gdef\@journalshort{Societies}\gdef\@doiabbr{soc}\gdef\@ISSN{2075-4698}}
\DeclareOption{socsci}{\gdef\@journal{socsci}\gdef\@journalfull{Social Sciences}\gdef\@journalshort{Soc. Sci.}\gdef\@doiabbr{socsci}\gdef\@ISSN{2076-0760}}
\DeclareOption{software}{\gdef\@journal{software}\gdef\@journalfull{Software}\gdef\@journalshort{Software}\gdef\@doiabbr{software}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{soilsystems}{\gdef\@journal{soilsystems}\gdef\@journalfull{Soil Systems}\gdef\@journalshort{Soil Syst.}\gdef\@doiabbr{soilsystems}\gdef\@ISSN{2571-8789}}
\DeclareOption{solar}{\gdef\@journal{solar}\gdef\@journalfull{Solar}\gdef\@journalshort{Solar}\gdef\@doiabbr{solar}\gdef\@ISSN{2673-9941}\gdef\@continuouspages{yes}}
\DeclareOption{solids}{\gdef\@journal{solids}\gdef\@journalfull{Solids}\gdef\@journalshort{Solids}\gdef\@doiabbr{solids}\gdef\@ISSN{2673-6497}\gdef\@continuouspages{yes}}
\DeclareOption{spectroscj}{\gdef\@journal{spectroscj}\gdef\@journalfull{Spectroscopy Journal}\gdef\@journalshort{Spectrosc. J.}\gdef\@doiabbr{spectroscj}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{sports}{\gdef\@journal{sports}\gdef\@journalfull{Sports}\gdef\@journalshort{Sports}\gdef\@doiabbr{sports}\gdef\@ISSN{2075-4663}}
\DeclareOption{standards}{\gdef\@journal{standards}\gdef\@journalfull{Standards}\gdef\@journalshort{Standards}\gdef\@doiabbr{standards}\gdef\@ISSN{2305-6703}\gdef\@continuouspages{yes}}
\DeclareOption{stats}{\gdef\@journal{stats}\gdef\@journalfull{Stats}\gdef\@journalshort{Stats}\gdef\@doiabbr{stats}\gdef\@ISSN{2571-905X}\gdef\@continuouspages{yes}}
\DeclareOption{std}{\gdef\@journal{std}\gdef\@journalfull{Surgical Techniques Development}\gdef\@journalshort{Surg. Tech. Dev.}\gdef\@doiabbr{std}\gdef\@ISSN{2038-9582}\gdef\@continuouspages{yes}}
\DeclareOption{stresses}{\gdef\@journal{stresses}\gdef\@journalfull{Stresses}\gdef\@journalshort{Stresses}\gdef\@doiabbr{stresses}\gdef\@ISSN{2673-7140}\gdef\@continuouspages{yes}}
\DeclareOption{surfaces}{\gdef\@journal{surfaces}\gdef\@journalfull{Surfaces}\gdef\@journalshort{Surfaces}\gdef\@doiabbr{surfaces}\gdef\@ISSN{2571-9637}\gdef\@continuouspages{yes}}
\DeclareOption{surgeries}{\gdef\@journal{surgeries}\gdef\@journalfull{Surgeries}\gdef\@journalshort{Surgeries}\gdef\@doiabbr{surgeries}\gdef\@ISSN{2017-2017}\gdef\@continuouspages{yes}}
\DeclareOption{suschem}{\gdef\@journal{suschem}\gdef\@journalfull{Sustainable Chemistry}\gdef\@journalshort{Sustain. Chem.}\gdef\@doiabbr{suschem}\gdef\@ISSN{2673-4079}\gdef\@continuouspages{yes}}
\DeclareOption{sustainability}{\gdef\@journal{sustainability}\gdef\@journalfull{Sustainability}\gdef\@journalshort{Sustainability}\gdef\@doiabbr{su}\gdef\@ISSN{2071-1050}}
\DeclareOption{symmetry}{\gdef\@journal{symmetry}\gdef\@journalfull{Symmetry}\gdef\@journalshort{Symmetry}\gdef\@doiabbr{sym}\gdef\@ISSN{2073-8994}}
\DeclareOption{synbio}{\gdef\@journal{synbio}\gdef\@journalfull{SynBio}\gdef\@journalshort{SynBio}\gdef\@doiabbr{synbio}\gdef\@ISSN{2674-0583}\gdef\@continuouspages{yes}}
\DeclareOption{systems}{\gdef\@journal{systems}\gdef\@journalfull{Systems}\gdef\@journalshort{Systems}\gdef\@doiabbr{systems}\gdef\@ISSN{2079-8954}}
\DeclareOption{targets}{\gdef\@journal{targets}\gdef\@journalfull{Targets}\gdef\@journalshort{Targets}\gdef\@doiabbr{targets}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{taxonomy}{\gdef\@journal{taxonomy}\gdef\@journalfull{Taxonomy}\gdef\@journalshort{Taxonomy}\gdef\@doiabbr{taxonomy}\gdef\@ISSN{2673-6500}\gdef\@continuouspages{yes}}
\DeclareOption{technologies}{\gdef\@journal{technologies}\gdef\@journalfull{Technologies}\gdef\@journalshort{Technologies}\gdef\@doiabbr{technologies}\gdef\@ISSN{2227-7080}}
\DeclareOption{telecom}{\gdef\@journal{telecom}\gdef\@journalfull{Telecom}\gdef\@journalshort{Telecom}\gdef\@doiabbr{telecom}\gdef\@ISSN{2673-4001}\gdef\@continuouspages{yes}}
\DeclareOption{test}{\gdef\@journal{test}\gdef\@journalfull{Test}\gdef\@journalshort{Test}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{textiles}{\gdef\@journal{textiles}\gdef\@journalfull{Textiles}\gdef\@journalshort{Textiles}\gdef\@doiabbr{textiles}\gdef\@ISSN{2673-7248}\gdef\@continuouspages{yes}}
\DeclareOption{thalassrep}{\gdef\@journal{thalassrep}\gdef\@journalfull{Thalassemia Reports}\gdef\@journalshort{Thalass. Rep.}\gdef\@doiabbr{thalassrep}\gdef\@ISSN{2039-4365}\gdef\@continuouspages{yes}}
\DeclareOption{thermo}{\gdef\@journal{thermo}\gdef\@journalfull{Thermo}\gdef\@journalshort{Thermo}\gdef\@doiabbr{thermo}\gdef\@ISSN{2673-7264}\gdef\@continuouspages{yes}}
\DeclareOption{tomography}{\gdef\@journal{tomography}\gdef\@journalfull{Tomography}\gdef\@journalshort{Tomography}\gdef\@doiabbr{tomography}\gdef\@ISSN{2379-139X}\gdef\@continuouspages{yes}}
\DeclareOption{tourismhosp}{\gdef\@journal{tourismhosp}\gdef\@journalfull{Tourism and Hospitality}\gdef\@journalshort{Tour. Hosp.}\gdef\@doiabbr{tourhosp}\gdef\@ISSN{2673-5768}\gdef\@continuouspages{yes}}
\DeclareOption{toxics}{\gdef\@journal{toxics}\gdef\@journalfull{Toxics}\gdef\@journalshort{Toxics}\gdef\@doiabbr{toxics}\gdef\@ISSN{2305-6304}}
\DeclareOption{toxins}{\gdef\@journal{toxins}\gdef\@journalfull{Toxins}\gdef\@journalshort{Toxins}\gdef\@doiabbr{toxins}\gdef\@ISSN{2072-6651}}
\DeclareOption{transplantology}{\gdef\@journal{transplantology}\gdef\@journalfull{Transplantology}\gdef\@journalshort{Transplantology}\gdef\@doiabbr{transplantology}\gdef\@ISSN{2673-3943}\gdef\@continuouspages{yes}}
\DeclareOption{transportation}{\gdef\@journal{transportation}\gdef\@journalfull{Transportation}\gdef\@journalshort{Transportation}\gdef\@doiabbr{transportation}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{traumacare}{\gdef\@journal{traumacare}\gdef\@journalfull{Trauma Care}\gdef\@journalshort{Trauma Care}\gdef\@doiabbr{traumacare}\gdef\@ISSN{2673-866X}\gdef\@continuouspages{yes}}
\DeclareOption{traumas}{\gdef\@journal{traumas}\gdef\@journalfull{Traumas}\gdef\@journalshort{Traumas}\gdef\@doiabbr{traumas}\gdef\@ISSN{2673-7477}\gdef\@continuouspages{yes}}
\DeclareOption{tropicalmed}{\gdef\@journal{tropicalmed}\gdef\@journalfull{Tropical Medicine and Infectious Disease}\gdef\@journalshort{Trop. Med. Infect. Dis.}\gdef\@doiabbr{tropicalmed}\gdef\@ISSN{2414-6366}}
\DeclareOption{universe}{\gdef\@journal{universe}\gdef\@journalfull{Universe}\gdef\@journalshort{Universe}\gdef\@doiabbr{universe}\gdef\@ISSN{2218-1997}}
\DeclareOption{urbansci}{\gdef\@journal{urbansci}\gdef\@journalfull{Urban Science}\gdef\@journalshort{Urban Sci.}\gdef\@doiabbr{urbansci}\gdef\@ISSN{2413-8851}}
\DeclareOption{uro}{\gdef\@journal{uro}\gdef\@journalfull{Uro}\gdef\@journalshort{Uro}\gdef\@doiabbr{uro}\gdef\@ISSN{2673-4397}\gdef\@continuouspages{yes}}
\DeclareOption{vaccines}{\gdef\@journal{vaccines}\gdef\@journalfull{Vaccines}\gdef\@journalshort{Vaccines}\gdef\@doiabbr{vaccines}\gdef\@ISSN{2076-393X}}
\DeclareOption{vehicles}{\gdef\@journal{vehicles}\gdef\@journalfull{Vehicles}\gdef\@journalshort{Vehicles}\gdef\@doiabbr{vehicles}\gdef\@ISSN{2624-8921}\gdef\@continuouspages{yes}}
\DeclareOption{venereology}{\gdef\@journal{venereology}\gdef\@journalfull{Venereology}\gdef\@journalshort{Venereology}\gdef\@doiabbr{venereology}\gdef\@ISSN{2674-0710}\gdef\@continuouspages{yes}}
\DeclareOption{vetsci}{\gdef\@journal{vetsci}\gdef\@journalfull{Veterinary Sciences}\gdef\@journalshort{Vet. Sci.}\gdef\@doiabbr{vetsci}\gdef\@ISSN{2306-7381}}
\DeclareOption{vibration}{\gdef\@journal{vibration}\gdef\@journalfull{Vibration}\gdef\@journalshort{Vibration}\gdef\@doiabbr{vibration}\gdef\@ISSN{2571-631X}\gdef\@continuouspages{yes}}
\DeclareOption{virtualworlds}{\gdef\@journal{virtualworlds}\gdef\@journalfull{Virtual Worlds}\gdef\@journalshort{Virtual Worlds}\gdef\@doiabbr{virtualworlds}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{viruses}{\gdef\@journal{viruses}\gdef\@journalfull{Viruses}\gdef\@journalshort{Viruses}\gdef\@doiabbr{v}\gdef\@ISSN{1999-4915}}
\DeclareOption{vision}{\gdef\@journal{vision}\gdef\@journalfull{Vision}\gdef\@journalshort{Vision}\gdef\@doiabbr{vision}\gdef\@ISSN{2411-5150}}
\DeclareOption{waste}{\gdef\@journal{waste}\gdef\@journalfull{Waste}\gdef\@journalshort{Waste}\gdef\@doiabbr{waste}\gdef\@ISSN{2813-0391}\gdef\@continuouspages{yes}}
\DeclareOption{water}{\gdef\@journal{water}\gdef\@journalfull{Water}\gdef\@journalshort{Water}\gdef\@doiabbr{w}\gdef\@ISSN{2073-4441}}
\DeclareOption{wem}{\gdef\@journal{wem}\gdef\@journalfull{Wildlife Ecology and Management}\gdef\@journalshort{Wildl. Ecol. Manag.}\gdef\@doiabbr{}\gdef\@ISSN{1234-4321}}
\DeclareOption{wevj}{\gdef\@journal{wevj}\gdef\@journalfull{World Electric Vehicle Journal}\gdef\@journalshort{World Electr. Veh. J.}\gdef\@doiabbr{wevj}\gdef\@ISSN{2032-6653}}
\DeclareOption{wind}{\gdef\@journal{wind}\gdef\@journalfull{Wind}\gdef\@journalshort{Wind}\gdef\@doiabbr{wind}\gdef\@ISSN{2674-032X}\gdef\@continuouspages{yes}}
\DeclareOption{women}{\gdef\@journal{women}\gdef\@journalfull{Women}\gdef\@journalshort{Women}\gdef\@doiabbr{women}\gdef\@ISSN{2673-4184}\gdef\@continuouspages{yes}}
\DeclareOption{world}{\gdef\@journal{world}\gdef\@journalfull{World}\gdef\@journalshort{World}\gdef\@doiabbr{world}\gdef\@ISSN{2673-4060}\gdef\@continuouspages{yes}}
\DeclareOption{youth}{\gdef\@journal{youth}\gdef\@journalfull{Youth}\gdef\@journalshort{Youth}\gdef\@doiabbr{youth}\gdef\@ISSN{2673-995X}\gdef\@continuouspages{yes}}
\DeclareOption{zoonoticdis}{\gdef\@journal{zoonoticdis}\gdef\@journalfull{Zoonotic Diseases}\gdef\@journalshort{Zoonotic Dis.}\gdef\@doiabbr{zoonoticdis}\gdef\@ISSN{2813-0227}\gdef\@continuouspages{yes}}


==> appliedsciences-twnet/supp_sections/abstract.tex <==
\begin{abstract}
This document provides supplemental material for \textit{\headline}.
\end{abstract}

==> conclusion.tex <==
\section{Conclusion}
	We present a novel framework TWNet for real-time high-resolution semantic video segmentation. % Our TWNet efficiently improves the performance and robustness of warping-based segmentation methods. 
	Specifically, we use warping and employ the non-key-frame CNN architecture for acceleration. 
In order to alleviate the errors caused by feature warping, we propose two efficient modules, namely CFR and RGA, to correct the warped features by learning the feature-space residual. Experimental results demonstrate that our method is much more robust than warping-based approaches while keeps the high speed.


==> experiment.tex <==
% We also conduct experiments to show that the refinement modules are able to alleviate error accumulation. 
\section{Experiments}
	In this section, we present the experimental results of TWNet on high-resolution videos. First, we introduce the experimental environment. Then, we perform ablation study to validate the effectiveness of the proposed non-key-frame CNN, CFR, and RGA. Finally, we compare TWNet with the state-of-the-art semantic video segmentation methods.

% Experimental Environment	
\subsection{Experimental Setup}

% dataset
\subsubsection{Dataset} 
	There are several commonly used datasets (e.g., Cityscapes \citep{cityscapes}, CamVid~\citep{camvid}, COCO-Stuff \citep{coco-stuff}, and ADE20K \citep{ade20k,zhou2019semantic}) for semantic segmentation. We perform training and evaluation on the Cityscapes dataset \citep{cityscapes} considering its high-resolution property and the requirements that the inputs should be video clips rather than images. Cityscapes contains 5000 high-resolution finely annotated images, which are divided into 2975, 500, and 1525 for training, validation and testing respectively. Each image is the $20^{th}$ frame of a $1024\times2048$ video clip. The dataset contains 19 classes for training and evaluation. 
	
	We perform the ablation study on the validation set of Cityscapes and compare the results of TWNet with the state-of-the-art methods. Also, we perform experiments on CamVid to demonstrate that our framework is generic to different datasets.

\subsubsection{Training} 
	% protocal 1. per-frame, 
	The training of TWNet is divided into two steps, i.e., the training of per-frame CNN and the training of the non-key-frame CNN.
	To train the per-frame model, we use the 2975 fine-annotated training images~(i.e., the $20^{th}$ frames in the video clips). We use MobileNet \citep{mobilenet} pre-trained on ImageNet~\citep{imagenet} as the encoder of the key-frame CNN, and use three cascaded lateral connections~\citep{fpn} as the decoder. We apply the Adam optimizer~\citep{adam} to train for $90K$ iterations with the initial learning rate of $1\times10^{-2}$ and batch size $8$. We update the pre-trained parameters with $100$ times smaller learning rate. Weight decay~$\lambda_0$ is set to $1\times10^{-7}$. Training data augmentations include mean extraction, random scaling between $0.5$ to $2.0$, random horizontal flipping, and random cropping to $[800, 800]$~($[600, 600]$ for CamVid). We implement the model using TensorFlow~1.12~\citep{tensorflow} and perform training on a single GTX~1080~Ti GPU card.
	
	% 2. warp-fcn(no crop)
	After the training of per-frame CNN, the parameters in it are fixed, and we start to train the non-key-frame CNN. In each training step of non-key-frame CNN, we first send a batch of the $19^{th}$ frames into the per-frame CNN to extract their context features. Then, we perform warping and correction for the corresponding $20^{th}$ frames and calculate the loss according to \cref{eq:loss2}. Note that if the consistency loss $\mathcal{L}_{consist}$ is employed, the $20^{th}$ frames should also be sent to the per-frame model to calculate the context features. In this training phase, random cropping is not adopted since the warping operation may exceed the cropped boundary. We set training size to $[1024, 2048]$~($[720, 960]$ for CamVid) with batch size 4. 
	% residual: pre-processing

\subsubsection{Evaluation} 
In the inference phase, we conduct all the experiments on video clips with the resolution of $1024\times 2048$. During evaluation, the key frame is uniformly sampled from the $9^{th}$ to the $20^{th}$ frame in the video clip, and the prediction of the $20^{th}$ frame is used for evaluation. No testing augmentation~(e.g., multi-scale or multi-crop) is adopted. The accuracy is measured by mean~Intersection-Over-Union~(mIoU), and the speed is measured by frames per second~(FPS). Our models run on a server with an Intel Core i9-7920X CPU and a single NVIDIA GeForce GTX 1080~Ti GPU card.

\subsection{Ablation Study}
	We start building TWNet from the training of the per-frame model. We adopt the commonly used lightweight CNN, MobileNetV1, as the encoder. Our per-frame model achieves the accuracy of $73.6\%$ mIoU at 35.5~FPS. %Results of \textbf{other backbones} and \textbf{lateral connection functions} are listed in the \textbf{supplemental material}.
%
%\begin{table}[t]
%\centering
%\begin{tabular}{lccc}
%\toprule
%Backbone CNN model &mIoU&FPS\\
%\midrule
%\midrule
%MobileNetV1&73.6&30.1\\
%MobileNetV2&73.2&26.7\\
%ResNet-18&72.1&31.2\\
%\bottomrule
%\end{tabular}
%\vspace{0.5em}
%\caption{Performance comparison of our modified per-frame FCN based on different backbones on Cityscapes val set.}
%\label{table:baseline}
%\end{table}	

% Ablation for warping-fcn
\subsubsection{The Non-Key-Frame CNN}
As described in Sec.~\ref{sec:warping-cnn}, in the non-key-frame CNN, the layer of feature maps can be arbitrarily chosen to balance the accuracy and speed. We choose three layers in the decoder as the context features respectively. Results are summarized in Table~\ref{table:warping-cnn}.

According the experimental results, fine-tuning~(the second training step) can significantly improve the performance. This demonstrates that low-level spatial features are more discriminative in the non-key-frame CNN, possibly due to the fact that the warped context features are less reliable in the non-key-frame CNN, thus the model depends more on low-level spatial features.
%in per-frame FCN, context feature is reliable and the network relies less on these low-level spatial features, while in Warp-FCN, the warped context feature is less reliable, thus the network depends more on  low-level spatial features.

\begin{table}[t]
\centering
\caption{Performance comparison of different layers used for interior warping. Interior warping: the layer of feature map used for interior warping; Fine-tuned: whether the second training step is performed to fine-tune the non-key-frame CNN. If not, the parameters of the head and tail layers keep the same as those in the per-frame CNN. If Layer~3 is chosen, there exists no trainable parameters and hence no fine-tuning.}
\label{table:warping-cnn}
\resizebox{0.42\textwidth}{!}{
\begin{tabular}{l|ccc}
\toprule
Warping Layer\ \  &\ Fine-tuned\ &\ mIoU\ &\ FPS\ \\
\midrule
\midrule
\multirow{2}{*}{Layer~1}&~&67.3&65.5\\
&$\checkmark$&69.6&65.5\\
\midrule
\multirow{2}{*}{Layer~2}&~&65.4&89.8\\
&$\checkmark$&67.8&89.8\\
\midrule
Layer~3&-&63.2&119.7\\
\bottomrule
\end{tabular}}
\end{table}	
%
\begin{table}[t]
\caption{Validation of $\mathcal{L}_{consist}$ during the training of CFR. $\lambda_1$: the weight of $\mathcal{L}_{consist}$.}
\label{table:cfr}
\centering
\resizebox{0.36\textwidth}{!}{
\begin{tabular}{l|ccc}
\toprule
Warping Layer\ \ &\ $\lambda_1$ \ & \ mIoU \ & \ FPS \ \\
\midrule
\midrule
\multirow{4}{*}{Layer~1}&0&69.9&63.1\\
&1&70.2&63.1\\
&10&\textbf{70.6}&63.1\\
&20&70.3&63.1\\
\midrule
\multirow{4}{*}{Layer~2}&0&67.6&86.3\\
&1&68.1&86.3\\
&10&\textbf{68.6}&86.3\\
&20&68.3&86.3\\
\bottomrule
\end{tabular}}
\end{table}	
% Ablation for refine module
\subsubsection{CFR Module and Consistency Loss}
	% wo kd vs kd
	We propose the CFR module to correct the warped context features. %by learning the residual in feature space. 
	As shown in Table~\ref{table:cfr}, the CFR module is effective and efficient. Table~\ref{table:cfr} also demonstrates the effectiveness of consistency loss, $\mathcal{L}_{consist}$, and the weight term, $\lambda_1$, a crucial hyper-parameter for the training of CFR. By default, we set $\lambda_1$ to 10 in the following sections for better performance.
%

% Ablation for residual-attention
\subsubsection{RGA Module}
	We introduce the RGA module to further exploit the correlation between residuals in image space and feature space. Results are demonstrated in Table~\ref{table:rga}. As expected, the RGA module further improves the performance of TWNet since it guides the CFR module to pay more attention to error-prone regions. The qualitative results of TWNet on Cityscapes are shown in Fig.~\ref{fig:qlt}.
%
\begin{table}[t]
\caption{Effect of each module of TWNet. FT: the fine-tuning of the non-key CNN~(the second training step); CFR: Context Feature Rectification; RGA: Residual-Guided Attention. ``$\checkmark$'' means the model utilizes the corresponding module.  We also show the extra cost of adding our modules.}
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|cccccc}
\toprule
Warping Layer \ \ & \ FT \ & \ CFR \ & \ RGA \ & \ mIoU \ & \ FPS \ & GFLOPs \\
\midrule
\midrule
\multirow{4}{*}{Layer~1}&&&&67.3&65.5 & 113.28\\
&$\checkmark$&&&69.6&65.5 & +0 \\
&$\checkmark$&$\checkmark$&&70.6&63.1 & +2.42\\
&$\checkmark$&$\checkmark$&$\checkmark$&\textbf{71.6}&61.8 & +0.0012\\
\midrule
\multirow{4}{*}{Layer~2}&&&&65.4&89.8 & 73.00\\
&$\checkmark$&&&67.8&89.8 & +0\\
&$\checkmark$&$\checkmark$&&68.6&86.3 & +2.42\\
&$\checkmark$&$\checkmark$&$\checkmark$&\textbf{69.5}&84.9 & +0.0029\\
\bottomrule
\end{tabular}}
\label{table:rga}
\end{table}	
%
%
\begin{figure*}[t]
\begin{center}
   	\includegraphics[width=1.0\linewidth]{qlt.pdf}
\end{center}
	\vspace{-1em}
   	\caption{Qualitative results on the Cityscapes dataset. GT: ground truth; Warping: normal warping; NKFC: the non-key-frame CNN; CFR: context feature rectification; RGA: residual-guided attention.}
\label{fig:qlt}
\end{figure*} 

\subsubsection{Category-Level Improvement}
	The IoU improvements for different categories are shown in Table~\ref{table:category}. The IoUs of \textbf{non-rigid objects}~(human, object and vehicle) are improved greatly because of the following reasons. Since the motions of these moving objects are hard to predict, thus, the warped results are inaccurate. Our correction modules correct the wrong predictions and thus improve the accuracy.
%
\begin{table*}[t]
\vspace{-1.0em}
\caption{IoU improvements of different categories. We choose Layer1 here.}
\centering
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{l|ccccccc}
\toprule
\small{Method}&\small{object}&\small{human}&\small{vehicle}&\small{nature}&\small{construction}&\small{sky}&\small{flat}\\
\midrule
\midrule
Warping
&43.8&56.7&82.2&86.6&87.1&91.6&96.6\\
NKFC~(The non-key-frame CNN)
&51.2~(+\textbf{7.4})&65.5~(+\textbf{8.8})&84.6~(+2.4)&89.6~(+3.0)&89.1~(+2.0)&94.0~(+2.4)&97.3~(+0.7)\\
NKFC + CFR
&62.2~(+\textbf{18.4})&75.2~(+\textbf{18.5})&89.7~(+\textbf{7.5})&91.3~(+4.7)&90.8~(+3.7)&94.2~(+2.6)&97.9~(+1.3)\\
NKFC + CFR + RGA
&62.2~(+\textbf{18.4})&76.1~(+\textbf{19.4})&90.1~(+\textbf{7.9})&91.1~(4.5)&91.0~(+3.9)&94.2~(+2.6)&98.0~(+1.4)\\
\bottomrule
\end{tabular}}
\label{table:category}
\end{table*}
%
%
\begin{figure*}[t]
\begin{center}
   	\includegraphics[width=0.98\linewidth]{error-accum.pdf}
\end{center}
	\vspace{-1.4em}
   	\caption{Performance degradation of Warp and Warp-Correct. (a): Layer~1 used for interior warping. (b): Layer~2 used for warping. $T$: frame interval between the key frame and the frame to be evaluated. The correction module effectively alleviates the long-term error accumulation problem.}
\label{fig:error-accum}
\end{figure*}
% robustness -> different interval between
%
\begin{table*}[t]
%\caption{Comparison of state-of-the-art semantic video segmentation models on Cityscapes. mIoU-pf: accuracy for per-frame model; FPS-pf: speed for per-frame model; mIoU: accuracy for video-based methods; FPS: speed for video-based methods. ``FPS~norm'' is calculated based on the performance of GPU. For previous works, we report the results in \textbf{the most comparable evaluation settings} to ours.}
\caption{Comparison of state-of-the-art semantic video segmentation models on Cityscapes. \textbf{Terms with ``-pf'': mIoU/FPS for per-frame model}; ``FPS~norm'' is calculated based on the performance of GPU. For previous works, we report the results in \textbf{the most comparable evaluation settings} to ours.}
\label{table:cmp}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccccccc}
\toprule
Model & \ train set \ & \ eval set \ & \ resolution \ & \ mIoU-pf \ & \ mIoU \ & \ FPS-pf \ & \ FPS \ & \ FPS norm \ & GPU\\
\midrule
\midrule
\multicolumn{2}{l}{\textit{Per-frame Models}}\\
ICNet~\citep{icnet}& train & val & $1024\times 2048$ & 67.7 & - & 30.3 & - & 49.7 & TITAN X(M)\\
ERFNet~\citep{erfnet}& train & test & $1024\times 2048$ & 69.7 & - & 11.2 & - & 18.4 & TITAN X(M)\\
%ICNet& train+val & test & 69.5 & $1024\times 2048$ & 30.3 & 49.7 & TITAN X(M)\\
%BiSeNet& train & val & 69.0 & $768\times 1536$ & 105.8 & 98.8 & TITAN Xp\\
SwiftNetRN-18~\citep{swiftnet}& train & val & $1024\times 2048$ & 74.4 & - & 34.0 & - & 34.0 & 1080~Ti\\
%DFANet & train & test & 71.3 & $1024\times 1024$ & 100.0 & 103.0 & TITAN X\\
CAS~\citep{cas}& train & val & $1024\times 2048$ & 74.0 & - & 34.2 & - & 48.9 & 1070\\
%CAS & train+coarse & val & 72.5 & $768\times 1536$ & 108 & 127.4 & 1070\\
%Ours~(modified FCN) & train & val & 73.6 & $1024\times 2048$ & 31.3 & 31.3 & 1080~Ti\\

\midrule
\midrule
\multicolumn{2}{l}{\textit{Video-based Models}}\\
DFF~\citep{dff}& train & val & $512\times 1024$ & 71.1 & 69.2 & 1.52 & 5.6 & 12.8 & Tesla K40\\
DVSNet1~\citep{dvsnet}& train & val & $1024 \times 2048$ & 73.5 & 63.2 & 5.6 & 30.4 & 30.4 & 1080 Ti\\
DVSNet2~\citep{dvsnet}& train & val & $1024 \times 2048$ & 73.5 & 70.4 & 5.6 & 19.8 & 19.8 & 1080 Ti\\
Prop-mv~\citep{jain2018fast}& train & val & $1024 \times 2048$ & 75.2 & 61.7 & 1.3 & 7.6 & 9.6 & Tesla K80\\
Interp-mv~\citep{jain2018fast}& train & val & $1024 \times 2048$ & 75.2 & 66.6 & 1.3 & 7.2 & 9.1 & Tesla K80\\
Low-Latency~\citep{low-latency}& train & val & $1024\times 2048$ & 80.2 & 75.9 & 2.8 & 8.4 & - & -\\

\midrule
\multicolumn{2}{l}{\textit{Ours}}\\
TWNet-Layer1& train & val & $1024\times 2048$ & 73.6 & 71.6 & 35.5 & 61.8 & 61.8 & \multirow{4}{*}{1080 Ti}\\
TWNet-Layer1& train & test & $1024\times 2048$ & 73.1 & 71.2 & 35.5 & 61.8 & 61.8 & \\
TWNet-Layer2& train & val & $1024\times 2048$ & 73.6 & 69.5 & 35.5 & 84.9 & 84.9 & \\
TWNet-Layer2& train & test & $1024\times 2048$ & 73.1 & 69.0 & 35.5 & 84.9 & 84.9 & \\
\bottomrule
\end{tabular}}
\end{table*}	
%

\subsubsection{Error Accumulation}
	We also conduct experiments to show that TWNet is able to alleviate the error accumulation problem during consecutive warping. Suppose $T$ denotes the frame-level interval between the initial key frame and the frame to be evaluated. We set $T$ to different values and evaluate the performance of TWNet and the non-key frame CNN without correction modules. Results in Fig.~\ref{fig:error-accum} show that the correction modules significantly alleviate the accuracy degradation and improve the robustness of the models. Meanwhile, the employment of CFR and RGA takes little extra time. 


\iffalse
\subsubsection{Choices of Feature Fusion} 
We study the effectiveness of different feature fusion functions and justify the choice.  We use lateral connections to fuse the low-level~(spatial) features with the high-level~(context) features. The manner of feature fusion is the same as that in FPN~(as shown in Fig.~\ref{fig:lateral}(a)), where the high-level feature maps are first upsampled by a  factor of two~(using bilinear interpolation) and then added by the low-level feature maps~(which goes through a $1\times 1$ convolution layer to align the channel dimension). We also perform experiments using the following variants: concatenation~(Fig.~\ref{fig:lateral}(b)) and conv-concatenation~(Fig.~\ref{fig:lateral}(c)). As demonstrated in Table~\ref{table:lateral}, our TWNet delivers consistent results for different fusion functions. Specifically, TWNet achieves better accuracy with conv-add fusion function and thus we use it in the paper.
%

\begin{figure*}[h]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=0.8\linewidth]{lateral.pdf}
\end{center}
	\vspace{-0.8em}
   \caption{ Different kinds of fusion functions. (a) Addition of two stacks of feature maps. (b) Concatenatiton of  two stacks of feature maps. (c) $1\times 1$ convolution for dimension alignment before concatenation.}
\label{fig:lateral}
\end{figure*}
%
\begin{table}[ht]
\caption{Comparison of different fusion functions for TWNet. We report results on the Cityscapes validation set. IW: the layer we use to do interior warping; None means no interior warping; mIoU: accuracy for video-based methods; FPS: speed for video-based methods. }
\label{table:lateral}
	\small
\centering
%\resizebox{\textwidth}{!}{
\begin{tabular}{llcccc}
\toprule
Fusion function 			& IW 	&  mIoU &  FPS & Speed-up ($\times$)\\
\midrule
\midrule
\multirow{3}{*}{\emph{conv-add}} 	& None~		& 73.6 	& 35.5 & -\\
					& Layer1	& 71.6 	& 61.8& 1.74\\
					& Layer2	& 69.5 	& 84.9& 2.39\\
\midrule
\multirow{3}{*}{\emph{concat}} 		& None~			& 73.3 	& 36.8 & -\\
					& Layer1		& 71.1  & 64.4	&  1.75\\
					& Layer2 		& 68.8  & 87.2	& 2.37\\
\midrule
\multirow{3}{*}{\emph{conv-concat}} 	& None~			& 74.0 	& 34.7 & - \\
					& Layer1		& 71.4	& 60.3& 1.74\\
					& Layer2 		& 69.2 	& 83.5& 2.41\\
\bottomrule
\end{tabular}
\end{table}	

\fi

\subsubsection{Choices of Backbones} 
We study the genericity of our TWNet to different backbones.  We show the results based on other lightweight backbones, i.e., MobileNetV2 and ResNet-18. 

As described in Section \ref{ssub:layer_selection}, we can choose different layers of the decoder for interior feature warping to create different versions of TWNet~(as illustrated in Fig.~\ref{fig:multi-layer}). Table~\ref{table:threelayers} shows the required \textit{head} layers for each version.


% \begin{figure}[h]
% \begin{center}
% %\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    \includegraphics[width=0.75\linewidth]{threelayers.pdf}
% \end{center}
% 	\vspace{-0.8em}
%    \caption{Choices of different layers for interior warping.}
% \label{fig:threelayers}
% \end{figure}

\begin{table}[ht]
\caption{The required \textit{head} layers for different versions of TWNet. head$n$: the $n^{th}$ \textit{head} layer of the encoder.}
\label{table:threelayers}
	\small
\centering
%\resizebox{\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
Model name & head1 & head2 & head3\\
\midrule
\midrule
Per-frame& $\checkmark$ & $\checkmark$ & $\checkmark$\\

TWNet-Layer1& $\checkmark$ & $\checkmark$ & \\

TWNet-Layer2& $\checkmark$ &  & \\

TWNet-Layer3&  &  &  \\
\bottomrule
\end{tabular}
%\vspace{0.8em}
\end{table}	

The head layers for different backbones are defined in Table~\ref{table:headlayers}. We use the notations from the TensorFlow Slim package.

\begin{table}[ht]
\caption{\textit{Head} layers for different backbones. We quote the notations from the TensorFlow Slim package.}
\label{table:headlayers}
	\small
\centering
%\resizebox{\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
Backbone & head1 & head2 & head3\\
\midrule
\midrule
MobileNetV1& $conv2d\_3$ & $conv2d\_5$ & $conv2d\_11$\\

MobileNetV2& $layer\_4$ & $layer\_7$ & $layer\_14$ \\

ResNet-18& $conv2\_2$ & $conv3\_2$ & $conv4\_2$ \\
\bottomrule
\end{tabular}
%\vspace{0.8em}
\end{table}
%
\begin{table}[ht]
\caption{Performance of TWNet based on different backbone networks. IW: the layer we use to do interior warping. ``None'' means no interior warping.}
\label{table:backbone}
	\small
\centering
%\resizebox{\textwidth}{!}{
\begin{tabular}{llcccc}
\toprule
	Backbone & IW & mIoU & FPS & Speed-up ($\times$)\\
\midrule
\midrule
	\multirow{4}{*}{MobileNetV1} & None & 73.6 & 35.5 & -\\
	&Layer1& 71.6 & 61.8 & 1.74\\
	&Layer2& 69.5 & 84.9 & 2.39\\
	&Layer3& 63.2 & 119.7 & 3.37\\

\midrule
	\multirow{4}{*}{MobileNetV2} & None & 73.2 & 32.3 & -\\
	&Layer1& 71.3 & 59.6 & 1.85\\
	&Layer2& 69.4 & 82.5 & 2.55\\
	&Layer3& 62.4 & 115.8 & 3.59\\

\midrule
	\multirow{4}{*}{ResNet-18} &  None & 71.6 & 36.9 & -\\
	&Layer1& 69.4 & 63.6 & 1.72\\
	&Layer2& 67.7 & 86.8 & 2.35\\
	&Layer3& 61.9 & 120.4 & 3.26\\

\bottomrule
\end{tabular}
\end{table}

Table~\ref{table:backbone} shows the experimental results of TWNet based on different backbones. 
In summary, TWNet is generic to backbone networks, and hence can be adapted to various per-frame models for different requirements of speed and accuracy.
% This means that our TWNet would achieve higher performance if a more delicate per-frame segmentation model were adopted.

\subsubsection{Choices of Flow Models}

We could use optical flow methods, e.g., FlowNet2~\citep{flownetv2} and PWC-Net~\citep{pwcnet}, as the flow model of our framework. However, the running speeds of these methods are even slower than our key-frame segmentation network (even slower than 20 fps), which means the warping operation will not speed up the inference phase. Also, when we use these optical-flow methods as warping, the segmentation accuracy is similar to our motion-vector version. Thus, we decide to use motion vectors. \cref{table:flow_models} shows the accuracy using different types of flows for warping.

\begin{table}[t]
\caption{Effect of different flow models.}
\label{table:flow_models}
\centering
%\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|cccc}
\toprule
Flow model \ \ 		& \ mIoU \	& \ FPS \  \\
\midrule
\midrule
Motion vectors		& 67.3 		& 65.5 \\
FlowNet2			& 67.5 		& 13.2 \\
FlowNet2-s  			& 66.3 		& 26.6 \\
FlowNet2-c  			& 66.6 		& 22.7 \\
PWC-Net   			& 67.0 		& 29.4 \\
\bottomrule
\end{tabular}%}
\end{table}	

\subsection{Comparison with Other Methods}
% Qualitative comparison(image)
	We compare the proposed TWNet with other state-of-the-art semantic video segmentation models, as shown in Table~\ref{table:cmp}. Note that the speed~(FPS) values measured in different models are just listed for reference, since the experimental environments may vary a lot. %Besides, some models reshape the input images to a lower resolution and some do not count the time of BN operations~\citep{bn}. 
	All of our models run on the platform with CUDA 9.2, cuDNN 7.3 and TensorFlow 1.12, and we use the \emph{timeline} tool in TensorFlow to measure the speed. Following the recent work of~\citep{swiftnet}, we include the ``FPS norm'' value based on the GPU types of previous methods~\footnote{GPU Benchmark:~\url{www.techpowerup.com/gpu-specs}}.
	%
	% relation with image-based methods
	Results demonstrate that our TWNet achieves the highest inference speed with comparable accuracy on inputs at a resolution of $1024\times 2048$. Also, the accuracy of TWNet decreases more slightly than other video-based methods. It is worth noting that we adopt the key-frame CNN to simplify our presentation. If a more delicate per-frame model were used, the performance of TWNet would be further improved.
%

	% FAIR!  FAIR!
	% Compare with other methods(big table)
\subsection{Results on the CamVid Dataset}
	We also conduct experiments on the CamVid dataset, which contains 367, 100, 233 $720\times 960$ video clips for training, validation and testing. We apply the same configurations as those of Cityscapes except for the crop size. As shown in \cref{table:camvid_ablation} and \cref{table:camvid_comparison}, TWNet achieves consistent results on CamVid. % For  comparison, our per-frame model achieves $73.5\%$ mIoU at 103.5 FPS.
%
\begin{table}[t]
\caption{Effect of each module of TWNet on the CamVid test set. }
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|ccccc}
\toprule
Warping Layer \ \ & \ FT \ & \ CFR \ & \ RGA \ & \ mIoU \ & \ FPS \ \\
\midrule
\midrule
\multirow{4}{*}{Layer~1}&&&&68.8&183.1\\
&$\checkmark$&&&69.9&183.1\\
&$\checkmark$&$\checkmark$&&71.0&179.8\\
&$\checkmark$&$\checkmark$&$\checkmark$&\textbf{71.5}&175.2\\
\midrule
\multirow{4}{*}{Layer~2}&&&&66.7&252.6\\
&$\checkmark$&&&68.1&252.6\\
&$\checkmark$&$\checkmark$&&69.3&245.8\\
&$\checkmark$&$\checkmark$&$\checkmark$&\textbf{70.0}&240.7\\
\bottomrule
\end{tabular}}
\label{table:camvid_ablation}
\end{table}	



\begin{table}[t]
\caption{Comparison with other methods on the CamVid test set. }
\label{table:camvid_comparison}
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|cccc}
\toprule
Model \ \ 						& \ mIoU-pf \ 	& \ mIoU \	& \ FPS-pf \ & \ FPS \  \\
\midrule
\midrule
DFANet A \citep{dfanet} 		& 64.7 			& - 		& 120		 & - \\
ICNet \citep{icnet} 			& 67.1			& - 		& 27.8 		 & - \\
BiSeNet \citep{bisenet} 		& 68.7 			& - 		& -			 & - \\
Prov-mv \citep{jain2018fast} 	& 68.6 			& 63.4 		& 3.8		 & 21.4 \\
Interp-mv \citep{jain2018fast}  & 68.6 			& 67.3 		& 3.8		 & 19.1 \\


\midrule
TWNet-Layer1 					& 73.5			& 71.5		& 103.5 	 & 175.2 \\
TWNet-Layer2 					& 73.5 			& 70.0 		& 103.5		 & 240.7 \\
\bottomrule
\end{tabular}}
\end{table}	

==> intro.tex <==
\section{Introduction}

%As an important and challenging problem in computer vision,
Semantic video segmentation aims at generating a sequence of pixel-wise class label maps for each frame in a video. 
A real-time solution to this task is challenging due to the stringent requirements of speed and space. Prevailing real-time methods can be grouped into two major categories: per-frame methods and warping-based methods.
%In general, there are two kinds of approaches.
Per-frame methods decompose the \emph{video} task into a stream of mutually independent \emph{image} segmentation tasks. They usually reduce the resolution of input images~\citep{segnet, dfanet, bisenet} or adopt a lightweight CNN \citep{mobilenet, dfanet, df1-seg, swiftnet, mobilenetv2, bisenet, cas, icnet} to meet the real-time demand. In light of the visual continuity between adjacent video frames, warping-based approaches~\citep{gadde2017semantic, jain2018fast, low-latency, dvsnet, dff} utilize some inter-frame motion estimation (e.g., optical flows~\citep{dvsnet, dff} or motion vectors~\citep{jain2018fast}) to avoid redundant computations, propagating (or \emph{warping}) the segmentation results from the previous frame to the current one. 

\begin{figure*}[t]
\begin{center}
   \includegraphics[width=0.9\linewidth]{warping-problem.pdf}
\end{center}
   \vspace{-1em}
	\caption{Qualitative results. The warped results are shown in the second row. (a)  Non-rigid moving objects suffer \textbf{deformation}. (b) Warping results in \textbf{error accumulation} along consecutive non-key frames. By adding the lightweight correction stage, these two kinds of problems are significantly alleviated as shown in the third row.}% All the inference settings are the same for (a) and (b).}
\label{fig:warping-problem}
\end{figure*}

Although existing warping-based methods significantly boost the inference speed by saving the computational time for numerous redundant frames, their performance drops considerably due to the following limitations.
\begin{inparaenum}[1)]
\item %\textbf{Overestimation}.
 % They lack the ability to preserve the local details. Namely, the motion information is often coarse-grained and hence imprecise for many small spatial regions.  
Every pixel in a non-key frame is estimated by motion flows from some pixels in the previous frame. Such estimation may work for continuous regions in a video, but the \emph{moving of a non-rigid object} such as a human usually becomes \textbf{severely deformed}, as shown in Fig.~\ref{fig:warping-problem}(a), since a non-rigid object in a new frame can contain a considerable amount of new pixels which cannot be estimated from the previous frame.
% (especially for non-rigid moving objects)
\item %\textbf{Error accumulations}.
\textbf{Errors accumulate} along consecutive non-key frames, making the results of later frames almost unusable, as shown in Fig.~\ref{fig:warping-problem}(b).
%It is worth noting that not only do inaccurate estimation errors from non-key frames but also segmentation errors from key frames contribute to error accumulation.
%They cannot handle the long-term error accumulation. 
%In the case of successive frames, the warping errors accumulate over time, 
\end{inparaenum}
All in all, warping behaves like a runaway fierce creature. The key to the issue is to tame it --- to take advantage of its acceleration and to keep it under control.


% We claim that these problems are caused since existing warping-based approaches lack the ability of self-correction.
%To alleviate inaccurate estimation errors and error accumulation, 
To deal with the issues above, we propose to introduce a lightweight correction stage after the warping stage, resulting in a novel framework, Tamed Warping Network~(TWNet), which contains a novel architecture and two correction modules for every non-key frame.
%(context feature refinement~(CFR) and residual-guided attention~(RGA)) to cope with error accumulation.
First, we propose the non-key-frame CNN~(NKFC) to perform segmentation for non-key frames. %preserve local details and empower later refinement in a warping-based manner. %and the refinement modules are applied to alleviate error accumulation. 
As shown in Fig.~\ref{fig:warping_strategy}, NKFC fuses warped deep features from a previous frame with the features from its shallow layers, making itself fast and able to retain spatial details, the requisites to do the following correction.
%It then fuses warped high-level context features with low-level spatial features, making the model fast and able to retain spatial details.
 %a small number of key frames (without warping) are fed into a vanilla segmentation network~(Fig.~\ref{fig:fcn}(a)). %, resulting in a set of feature maps associated with different network layers.
%For the rest part of frames~(non-key frames), we adopt a Warping-CNN~(Fig.~\ref{fig:fcn}(b)) architecture to perform segmentation. On the one hand, we apply interior warping to obtain the high-level context features. On the other hand, we preserve several \emph{head} and \emph{tail} layers of the segmentation CNN to extract low-level spatial features and fuse the two kinds of features, making the Warping-CNN able to retain spatial details.
%only the low-level features for the non-key frames (to the warped) are extracted to represent their corresponding local detail information.
%As shown in Fig.~\ref{fig:fcn},interior feature warping directly warps the intermediate high-level feature maps onto the non-key frames (instead of the final segmentation results), resulting in their corresponding warped high-level features.
%Subsequently, it learns a fusion module to incorporate the low-level features into the warped high-level features, leading to the local-detail-preserving features for segmentation prediction. 
%To cope with error accumulation, 
To alleviate the issue of deformation, we introduce a correction stage consisting of two modules. We design the context feature rectification~(CFR) module to correct the warped features with the help of spatial details contained in NKFC.  To help CFR focus on error-prone regions, we design the residual-guided attention~(RGA) module to utilize the \textit{Residual Maps} in the compressed domain. It is worth noting that TWNet alleviates error accumulation in that it corrects every non-key frame rather than indulging the warping without restriction.
% distance  the residual in feature space.
%we design the CFR module to correct the errors caused by feature warping by learning the feature-space residual.
% Inspired by the video codecs (e.g., MPEG~\cite{mpeg} or H.264~\cite{h264}), where the warped image requires an additional \emph{residual map} for correction, we propose to refine the warped feature by learning the feature-space residual. %The CFR module   and generates a set of residual feature maps working as compensation features, which are added to the warped feature maps (associated with the non-key frames) for correction. 
%To further guide the learning process of CFR, we propose the RGA module, which utilizes the image-space residual from the compress domain as the attention weights.
%Consequently, the refinement modules effectively alleviate the error accumulation problem.

\begin{figure*}[t]
\begin{center}
   	\includegraphics[width=0.75\linewidth]{fpn.pdf}
\end{center}
	\vspace{-1em}
	\caption{(a) Commonly-used warping-based approaches. (b) Our TWNet. Black arrows denote the main path of the network, while gray arrows denote the lateral connections~\citep{fpn}. The warped layers are indicated by red color. The dotted arrows and boxes denote skipped operations.}% the part which need not to be calculated.} %for non-key frames.}
\label{fig:warping_strategy}
\end{figure*}
	
We evaluate TWNet on the Cityscapes~\citep{cityscapes} and CamVid~\citep{camvid} datasets. 
Experimental results show that TWNet greatly improve the accuracy and robustness of warping-based models. Specifically, for the $1024\times 2048$ videos on Cityscapes, the accuracy~(mIoU) significantly increases from $67.3\%$ to $71.6\%$ by adding the correction, and the speed edges down from 65.5 FPS to 61.8 FPS. Furthermore, we found the performance improvements of non-rigid categories such as ``human'' and ``object'' are even higher than 18 percentage points.

%Both of the versions achieve state-of-the-art accuracy among warping-based approaches.


The main contributions of this work are summarized as follows:
\begin{itemize}
\item
	We propose a novel framework, Tamed Warping Network~(TWNet), to improve the performance of warping-based segmentation models by introducing a light-weight correction stage.
%\item
%	We propose the Warping-CNN architecture with the warping strategy to speed up segmentation while preserve spatial details. %, which adopts interior feature warping and fuses the warped context features with the extracted spatial features, aiming to speed up while preserve spatial details.%, aiming to generate the local-detail-preserving warped context features. 
\item
    We propose two efficient correction modules, the Context Feature Rectification module as well as the Residual-Guided Attention module, to alleviate the non-rigid object deformation and error accumulation problems during feature warping.
    % , to correct the warped context feature by learning the feature-space residual, aiming to alleviate the error accumulation problem during successive feature warping.
\item
    Experimental results on Cityscapes and CamVid demonstrate that the proposed TWNet framework greatly improves the robustness and accuracy.
\end{itemize}








	
	


	


==> method.tex <==
\section{Tamed Warping Network}
\label{sec:methods}

	In this section, we introduce the Tamed Warping Network~(TWNet).
	%We start by introducing the inter-frame prediction process in video codecs, which inspires us to design the refinement modules.
	We first outline the overall framework.
	Next, we introduce our non-key-frame CNN architecture and the correction modules, i.e., the Context Feature Rectification~(CFR) module as well as the Residual-Guided Attention~(RGA) module. 
%In the refinement stage, we describe the Context Feature Refinement~(CFR) module as well as the Residual-Guided Attention~(RGA) module. 
	Finally, we present the implementation details. 
	%Next, we introduce the key modules of WRNet, including the basic networks structure, Warp-FPN, the Context Feature Refinement~(CFR) module, and the Residual-Guided Attention~(RGA) module. Finally, implementation details are presented. 
		

% Overview
\subsection{Overview}

\begin{figure*}[t]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=1.0\linewidth]{wrnet.pdf}
\end{center}
	\vspace{-0.8em}
   \caption{ The framework of Tamed Warping Network. The key-frames~(I-frames) are sent to the key-frame CNN. The non-key frames (P-frames) are sent to the non-key-frame CNN, where the warped context features are first corrected by the CFR and RGA modules and then fused with the spatial features extracted from the current frame. Both branches output the  result label maps and the interior context feature maps.}
\label{fig:wrnet}
\end{figure*}

	The whole framework of Tamed Warping Network~(TWNet) is illustrated in~Fig.~\ref{fig:wrnet}. In our framework, video frames are divided into key frames~(I-frames) and non-key frames (P-frames). The key frames are sent to the key-frame CNN (an U-shape~\citep{fpn, unet} FCN) where the context features of a selected interior layer are sent~(warped) to the next frame. For non-key frames, the warped features are first corrected by the Context Feature Rectification~(CFR) and Residual-Guided Attention~(RGA) modules and then fused with the spatial features of the current frame. 
	% the Warping-CNN receives the context features from the previous frame, which is fused with currently-extracted spatial feature using the Context Feature Refinement~(CFR) and Residual-Guided Attention~(RGA) modules for correction.
Then, the resultant features are used to make prediction and also sent to the next frame. The components of TWNet are described as follows. %in the following part.
	



\subsection{Basic Model: The Non-Key-Frame CNN}
\label{sec:warping-cnn}

	% featire warping
	Warping can be applied in feature space~(Fig.~\ref{fig:inter-frame}(b)) since the ``conv'' layers in FCN models preserve the position information. Given the features of the previous frame $\mathcal{F}_{t-1}$, we can use $Mv_{t}$ to predict the features of the current frame $\hat{\mathcal{F}}_{t}$ by 
%
\begin{equation}
\begin{split}
	\mathcal{\hat{F}}_t = \mathrm{warp}(\mathcal{F}_{t-1}, Mv_{t}).
\end{split}
\label{eq:wocfr}			
\end{equation}

\begin{figure*}[tb]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=0.7\linewidth]{cfr-rga.pdf}
\end{center}
	\vspace{-0.8em}
   \caption{Details of (a)~CFR and (b)~CFR+RGA. ``$\odot$'': element-wise multiplication; ``$+$'': element-wise addition. }
\label{fig:cfr-rga}
\end{figure*}

	%

	%In this work, we propose the architecture, Warping-CNN using the feature warping strategy. Compared with the vanilla segmentation CNN, Warping-CNN preserves several \emph{head} and \emph{tail} layers of the segmentation CNN. The \emph{head} layers extract low-level spatial features while  \emph{tail} layers fuse the spatial features by lateral connections. Meanwhile, we use feature warping to estimate the high-level context feature maps of the current non-key frame, as shown in Fig.~\ref{fig:wrnet}. % as well as the warped context features.

	%Warping-CNN takes into account both efficiency and accuracy.
	In this work, we propose the non-key-frame CNN architecture as the basic model to perform segmentation for non-key frames considering both efficiency and accuracy. For one thing, in order to speed up, it applies interior warping to obtain deep context features. For another, different from previous warping methods, the non-key-frame CNN preserves several shallow \emph{head} layers to add spatial features. Then, the two kinds of features are fused by lateral connections as FPN~\citep{fpn} and U-Net~\citep{unet}. Meanwhile, it is worth noting that the spatial features are also provided to the correction modules as the input.

% As for the key-frame CNN, the non-key-frame CNN without interior warping from a previous frame becomes the key-frame CNN, as shown in Fig.~\ref{fig:wrnet}.

	%Previous works~\cite{swiftnet, bisenet, cfnet} have shown that context features play an important role in semantic segmentation, but it is usually time-consuming to extract context features since they usually lie in deeper layers of the network. In order to reduce the computations, Warping-CNN obtains the context features by feature warping. Considering the fact that feature warping may lose detailed information since motion vectors are weak in spatial details~(as shown in Fig.~\ref{fig:inter-frame}), %we preserve several \emph{head} and \emph{tail} layers of the segmentation CNN to extract spatial features and fuse two kinds of features by lateral connection. 
%we preserve several \emph{head} layers of the segmentation CNN to extract spatial features. 

	% 2 aspects.  1. the context feature resolution low, 
	
	% Feature fusion. context + sptail for details compensation
\subsection{The Correction Stage}
\label{sec:cfr}
	 
	
	Inspired by this correction step in video codecs, we propose to add a correction step~(right part of Fig.~\ref{fig:inter-frame}(b)) in our segmentation pipeline. %to correct the warped feature by learning the \textit{residual} term in feature space using a context feature refinement~(CFR) module. 
	%$Besides, observing the spatial consistency between image space and feature space, we propose to use the residual map in image space to guide the learning of CFR in an attention manner. %by employing a residual-guided attention~(RGA) module.
	%
	The correction stage consists of two key modules. The Context Feature Rectification~(CFR) module corrects the warped features, and the Residual-Guided Attention~(RGA) module guides the learning of CFR.
	
	% 显示进行 refine
\subsubsection{Context Feature Rectification}
	Although the non-key-frame CNN can add spatial details by employing low-level features via lateral connections, still, the errors in context feature would accumulate during successive feature warping. Thus, we claim the warped context features themselves need to be corrected.
	Comparing the pipeline of video codecs with warping-based segmentation methods~(Fig.~\ref{fig:inter-frame}), we find the main problem of previous methods is the lack of a correction stage, which leads to inaccurate predictions and the error accumulation issue. 
	
	Inspired by the correction step in video codecs, we introduce the lightweight Context Feature Rectification~(CFR) module to explicitly correct the warped context features. 
	We design the CFR module considering the following aspects. First, the contextual information of the warped features is generally correct, except for the \textit{edges of moving objects}. Second, the low-level features contain the spatial information, such as ``edge'' and ``shape''. Thus, we claim the shape information in low-level features can help to correct the context feature, and we apply feature aggregation to perform this correction.
	CFR takes the warped context features $\hat{\mathcal{F}}_{t}$ as well as the spatial features of the current frame $f_t$ as the inputs and outputs the corrected context features $\mathcal{F}_t$, as shown in Fig.~\ref{fig:cfr-rga}(a). Specifically, the CFR module adopts a single-layer network, $\phi_r$, which takes the concatenation $[\hat{\mathcal{F}}_{t}$, $f_t]$ as the input and outputs the residual in feature space, $Res\mathcal{F}_t$. The mathematical form of CFR is defined as
%
\begin{equation}
\begin{split}
	\mathcal{F}_t &= \hat{\mathcal{F}}_{t} + \phi_{r}([\hat{\mathcal{F}}_{t}, f_t])\\
	&=  \mathrm{warp}(\mathcal{F}_{t-1}, Mv_{t}) + Res\mathcal{F}_t.
\end{split}
\label{eq:withcfr}			
\end{equation} 
%
%
	During the training of CFR, in addition to the commonly used softmax cross entropy loss $\mathcal{L}_{cls}$ for pixel-level classification, we propose to employ an L2 consistency loss $\mathcal{L}_{consist}$ to minimize the distance between the corrected context features and the features extracted by the per-frame CNN.% We add this consistency loss since we expect the output of Warp-FCN is as similar as that of the per-frame FCN. 




\subsubsection{Residual-Guided Attention}
%\subsection{Residual-Guided Attention}
	% consistency
	To guide the learning of CFR and further improve its performance, we propose the Residual-Guided Attention~(RGA) module.
	
	In our TWNet, the motion vectors used for feature warping are the same as those used in image warping. Therefore, the \textit{biases/errors should appear in the same spatial regions} in image space and feature space. Thus, the residual maps in image space $ResI_t$ can be used as prior information to guide the learning of residuals in feature space $Res\mathcal{F}_t$. To realize this guidance, we adopt a lightweight spatial attention module named RGA to let the CFR module focus more on the regions with higher responses in $ResI_t$. 
	%In above sections, we apply warping in feature space using the motion vectors extracted from image space. This works since these two spaces are spatially consistent~(mainly because operations in CNN preserve the spatial structure). We claim this consistency also holds for \textit{residuals} in these two spaces, which means high response should appear in the same spatial regions in these two kinds of \textit{residuals}. Based on this, we propose the RGA module to guide the learning of CFR by fully exploiting the prior spatial information contained in residuals from image space.
	Specifically, we first resize the residual map~$ResI_t$ to the shape of the warped context features. Then, we calculate the spatial attention map~$\mathcal{A}_t$ using a single-layer feed-forward CNN~$\phi_a$ as follows
%
\begin{equation}
\begin{split}
	\mathcal{A}_t &= \phi_a(ResI_t).
\end{split}
\label{eq:attention}			
\end{equation}
	Finally, we apply spatial attention by performing element-wise multiplication between $\mathcal{A}_t$ and $Res\mathcal{F}_t$. Fig.~\ref{fig:cfr-rga}(b) illustrates the detailed structure of RGA. After applying this module, %we obtain Eq.~\ref{eq:wrnet}, which gives the whole process of the proposed WRNet for non-key frames.
we formulate the whole process of TWNet for non-key frames, defined as 
%
\begin{equation}
\begin{split}
	\mathcal{F}_t &= \hat{\mathcal{F}}_{t} + \mathcal{A}_t\odot Res\mathcal{F}_t.
\end{split}
\label{eq:wrnet}			
\end{equation} 


\subsection{Implementation Details}
	%In this section, we describe the implementation details of WRNet.

% key/non-key decison: I-frame, P-frame, compressed domain
\subsubsection{Motion Extraction and Key Frame Selection} 
In our TWNet, we utilize \textit{motion vectors} as motion maps. Both \textit{motion vectors} and \textit{residuals} are already contained in compressed videos. Thus, it takes no extra time to extract them. As for key frame scheduling, we simply regard all I-frames as key frames and P-frames as non-key frames, where I/P-frames are  the concepts in video compression. An I-frame~(Intra-coded picture) is stored as a complete image, while a P-frame~(Predicted picture) is stored by the corresponding motion vectors and residual. Following previous works of~\citep{dmcnet, coviar}, we choose MPEG-4~Part~2~(Simple Profile)~\citep{h264} as the compression standard, where each group of picture~(GOP) contains an I-frame followed by 11 P-frames.

% changable layer
\subsubsection{Layer Selection in the Non-Key-Frame CNN}\label{ssub:layer_selection}
	It is worth noting that the layer of feature map used for warping can be arbitrarily chosen. In general, if we choose a deeper layer, there will be less corresponding \textit{head} and \textit{tail layers}~(Fig.~\ref{fig:multi-layer}), since layers in the encode-decoder architecture are paired by lateral connections. Thus, we will obtain a faster while less accurate model. Practically, we can adjust this hyperparameter to strike a balance between speed and accuracy. 
%
\begin{figure}[t]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=0.98\linewidth]{multi-layer.pdf}
\end{center}
	\vspace{-0.8em}
   \caption{ Choices of different layers for interior warping. The chosen layer is indicated with red color. The dotted arrows and boxes denote skipped operations.}
\label{fig:multi-layer}
\end{figure}
% warp-fpn
%\noindent \textbf{Details of Warp-FCN:} 
%	% backbone:	2 different
%We start building WRNet from the design of modified FCN and Warp-FCN. We choose the commonly used lightweight CNN backbone, MobileNet~\cite{mobilev1}, as the encoder of FCN. In the decoder phase, we employ three upsampling stages, where the first upsampled layer is treated as the context layer by default. We use the same lateral connection as described in original FCN~\cite{fpn}. Before the warping phase, the motion vector is resized to the shape of the corresponding feature map.



	
% weight of different losses
\subsubsection{Training of TWNet}
	In general, the training of TWNet contains two main steps, i.e., the training of the per-frame CNN and the training of the non-key-frame CNN. The training of the per-frame CNN is similar to that of other image segmentation methods, where  the softmax cross entropy loss~$\mathcal{L}_{cls}$ and the regularization loss~$\mathcal{L}_{reg}$ are used.
%%
%\begin{equation}
%\begin{split}
%	\mathop{\arg \min}_{\theta_0}~~\mathcal{L}_{cls} + \lambda_0\mathcal{L}_{reg},
%\end{split}
%\label{eq:loss1}			
%\end{equation} 
%%
%	where $\theta_0$ contains trainable parameters in the modified FCN.
	Then, we fix all the parameters in the per-frame model~(the key-frame CNN) and start to train the modules in the non-key-frame CNN. As mentioned in Sec.~\ref{sec:cfr}, we employ an additional L2 consistency loss $\mathcal{L}_{consist}$ to minimize the distance between the corrected features and the context features extracted from the key-frame CNN. The object function of this training step is defined as
%
\begin{equation}
\begin{split}
	%\mathop{\min}~~
	\mathcal{L} = \mathcal{L}_{cls} + \lambda_0\mathcal{L}_{reg} + \lambda_1\mathcal{L}_{consist},
\end{split}
\label{eq:loss2}			
\end{equation} 
%	
	where $\lambda_0$ and $\lambda_1$ are weights to balance different kinds of losses.
	
	During inference, we leave out the consistency loss since only one path~(i.e., either the key-frame CNN or non-key-frame CNN) is used.
	
	% warping resolution
	
	% little difference: we only utilize the last layer to predict the label



%\subsection{Warp-FPN}
%	% Warp
%	We first describe the basic structure, Warp-FPN, of our WRNet. As shown in~Fig.~\ref{fig:fpn} and~Fig.~\ref{fig:wrnet}, in Warp-FPN, only low-level spatial features will be extracted by CNN. While for context feature, instead of extracting it through the main path of CNN, we use feature warping to obtain it. Given the context feature of previous frame, $\mathcal{F}_{t-1}$, and the current motion vector, $Mv_{t}$, the feature warping to predict $\hat{\mathcal{F}}_{t}$ is defined by
%	%
%\begin{equation}
%\begin{split}
%	\hat{\mathcal{F}}_{t}(p) &= \mathcal{F}_{t-1}(p-Mv_{t}(p)),
%\end{split}
%\label{eq:feature-warp}			
%\end{equation} 
%	where $p\in R^{H\times W}$ is the index of feature map.
%	We design the Warp-FPN considering both efficiency and accuracy.
%	Previous works~\cite{bise, ic, swift} have shown that context features play an important role in semantic segmentation. However, it is usually time-consuming to extract context features since they are high-level features from deeper layers of CNN. In order to reduce the heavy computations, the Warp-FPN obtain the context feature by feature warping, which is a lightweight operation. However, feature warping may introduce noise since motion vectors are not good at dealing with spatial details~(as shown in Fig.~\ref{fig:flow-mv}). Therefore, the Warp-FPN preserves several initial layers of CNN to extract spatial features and it fuses two kinds of features by lateral connection, which is the same as that in a normal FPN. 
%	
%	%First, we analyze the segmentation quality. On the one hand, previous approaches~\cite{bise, ic, swift} has shown that features from deeper layers contain more context information and they are less sensitive to local changes, while features from shallower levels capture more spatial details. On the other hand, motion vectors can generally predict the global movements well, while they are not good at dealing with spatial details. %Thus, it is more suitable to warp the context feature. 
%	%Second, when considering the speed, the computations of context feature extraction are much heavier compared with that of warping, while the time for warping and spatial feature extraction are s. 
%	%Therefore, the proposed Warp-FPN preserves the extraction of spatial feature while uses warping to obtain context feature, which naturally fits the structure of FPN.
%	% 2 aspects.  1. the context feature resolution low, 
%	
%	% Feature fusion. context + sptail for details compensation
%\begin{figure}[t]
%\begin{center}
%%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%   \includegraphics[width=0.99\linewidth]{images/multi-layer.pdf}
%\end{center}
%	\vspace{-1em}
%   \caption{ Choose different layers as the \textit{context layer} results in different models. The context feature map is indicated with red color. The dotted line denotes the part which need not to be calculated.}
%\label{fig:multi-layer}
%\end{figure}
%	% changable layer
%	It is worth noting that the \textit{context layer} can be arbitrarily chosen. In general, if we choose to warp the later layer, there will be less corresponding \textit{spatial layers}~(Fig.~\ref{fig:multi-layer}), and thus we will obtain a less accurate while faster model. Practically, we can adjust this parameter to achieve the balance between accuracy and speed. 


==> prelim.tex <==
\section{Preliminaries: Warping and Correction in Video Codecs}
\label{sec:prelim}

\begin{figure*}[t]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=0.9\linewidth]{inter-frame.pdf}
\end{center}
	\vspace{-0.8em}
   \caption{ Visualization of \textbf{Warping} and \textbf{Correction}. (a) In image space, video codecs first warp the previous frame to the current  one, then add the image-space residual map for correction. (b) We propose to learn the \textbf{residual in feature space} to rectify the warped features. Note that for better visualization, we use segmentation labels to represent features.}
\label{fig:inter-frame}
\end{figure*}

	In this section, we describe the basics and the pipeline of warping-correction%~(Fig.~\ref{fig:inter-frame}(a)) 
in video codecs.
	% warping
	Warping is an efficient operation for inter-frame prediction. Given the previous frame $I_{t-1}$ and the motion vectors of the current frame $Mv_t$, we can estimate the current frame $\hat{I}_t$ by image warping. The process is described as
\begin{equation}
\begin{split}
	\hat{I}_t = \mathrm{warp}(I_{t-1}, Mv_t).
\end{split}
\label{eq:warp}			
\end{equation}
%
For a particular location index $p\in \mathcal{Z}^{H\times W}$ in an image, the mapping function is given by
	%
\begin{equation}
\begin{split}
	\hat{I}_{t}[p] &= I_{t-1}[p-Mv_{t}[p]].
\end{split}
\label{eq:feature-warp}			
\end{equation}

	% Residual
	However, there always exist biases between the warped image and the real one, especially in some complicated scenes and for the non-rigid moving objects. In order to correct the biases in image space, modern video codecs~(e.g., MPEG~\citep{mpeg}, H.264~\citep{h264}) add a correction step after image warping~(Fig.\ref{fig:inter-frame}(a)). 
	Specifically, the codec performs pixel-wise addition between the warped image $\hat{I}_t$ and the \textit{residual map} $ResI_t$ to make correction. Each point in $ResI_t$ is a three-dimensional vector, $(\Delta r, \Delta g, \Delta b)$, which describes the color differences between the warped pixel and the expected one. The overall inter-frame prediction process is described as
		%the inter-frame prediction~(\ie, motion compensation) usually contains two steps. First, the codec performs image warping using motion vectors. After that, pixel-wise addition between the warped image~(may contain error) and the residual map is performed for correction. Let $X_t$ denotes the $t^{th}$ frame. $Mv_t$, $Res_t$ are the corresponding motion vector and residual, the prediction process is described as
\begin{equation}
\begin{split}
	I_t &= \mathrm{warp}(I_{t-1}, Mv_t) + ResI_t.
\end{split}
\label{eq:warp-refine}			
\end{equation}
%
	%The key difference between Eq.~\ref{eq:warp} and Eq.~\ref{eq:warp-refine} is that the codec adds a residual term for correction. 
	The correction step effectively addresses the bias problem and the error accumulation problem in image space. Inspired by this, \textbf{we propose to learn the residual term in feature space}~(Fig.~\ref{fig:inter-frame}(b)) to alleviate problems incurred by feature warping.

		 
		
		


==> related.tex <==
\section{Related Work}
\label{sec:related}
%	Driven by the development of deep convolutional neural networks~(DCNNs), 
	

%Real-time methods usually reduce the scale of input images or adopt lightweight networks (either a lightweight backbone or a customized lightweight architecture). In this work, we %utilize temporal continuity in video by warping and minimize its resulting errors by feature fusion. Next, we briefly summarize these two aspects.
	%In this section, 
% (either a light-weight CNN backbone, \eg, ResNet18~\cite{resnet} and MobileNet~\cite{mobilenet, mobilenetv2}, or a custom lightweight architecture~\cite{df1-seg, cas})
\subsection{Feature Fusion in Semantic Segmentation}
	% Segmentation
Semantic segmentation in an FCN manner~\citep{fcn} has achieved remarkable accuracy. Recently, high-quality models~\citep{deeplabv3+, ccnet, cfnet, pspnet, ann, danet, dynamic-filter} %, such as PSPNet~\cite{pspnet}, DeeplabV3+~\cite{deeplabv3+}, and CFNet~\cite{cfnet}
as well as high-speed lightweight approaches~\citep{dfanet, swiftnet, bisenet, icnet} %, such as ICNet~\cite{icnet}, BiSeNet~\cite{bisenet}, DFANet~\cite{dfanet} and SwiftNet~\cite{swiftnet}, 
show the importance of feature fusion from different layers~(or scales). Generally, shallow layers contain more low-level \textit{spatial} details, while deep layers more \textit{contextual} information. The combination of features from different layers significantly improve the accuracy.
	
	% Relation
	Feature fusion in our proposed non-key-frame CNN is similar to those in FPN~\citep{fpn} and U-Net~\citep{unet}, where lateral connections are used to fuse the low-level~(spatial) and high-level~(context) features. 
%	The main difference between these two methods and 
In comparison, our non-key-frame CNN only retains a small number of layers of the encoder to extracts low-level features and obtains high-level features by interior feature warping. % , while high-level features are obtained by feature warping. %warping the context features from the previous frame.
Thus, the non-key-frame CNN saves the heavy computations of context feature extraction.
	
	% Features in videos
	\vspace{1em}
\subsection{Warping-Based Video Segmentation}
	In general, videos are of temporal continuity, i.e., consecutive video frames look similar,  
	% In videos, consecutive frames are strongly correlated~(\ie, they look similar in appearance), 
	making it possible to perform inter-frame prediction. The process of mapping pixels from the previous frame to the current one according to a pixel-level motion map is called image warping~(Fig.~\ref{fig:inter-frame}). 
	%Suppose the resolution of a video clip is $H\times W$, then motion map is with the shape of $H\times W \times 2$, where each point, $(\Delta x, \Delta y)$, 
	Each point in the motion map is a two-dimensional vector, $(\Delta x, \Delta y)$, representing the movement from the previous frame to the current one. Motion vectors and optical flows are two kinds of commonly used motion maps. In general, motion vectors, already contained in videos, are less precise than optical flows~(e.g., TV-L1~\citep{tv-l1} FlowNet2.0~\citep{flownetv2} and PWC-Net~\citep{pwcnet}). However, it takes extra time to perform optical flow estimation. 
	
%\begin{figure}[tb]
%\begin{center}
%%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%   \includegraphics[width=0.95\linewidth]{images/flow-mv.pdf}
%\end{center}
%	\vspace{-1em}
%   \caption{Different kinds of motion maps. We convert the 2D motion values into 3D HSV values, where hue and saturation refer to the direction~(angle) and magnitude of the motion respectively. In general, both motion vectors and optical flow fields can correctly represent most kinds of movements. Optical flow fields contain more details at the original resolution, while movements of objects are more consistent in motion vectors~(e.g. we can see the shape of cars in motion vectors). }
%\label{fig:flow-mv}
%\end{figure}

	% warping
	Researchers have proposed many warping-based semantic video segmentation approaches~\citep{gadde2017semantic, jain2018fast, dvsnet, dff}. Gadde~et al.~\citep{gadde2017semantic} proposed to enhance the features of the current frame by adding it with the warped features from previous frames. Zhu~et al.~\citep{dff}, Xu~et al.~\citep{dvsnet} and Jain~et al.~\citep{jain2018fast} proposed to use feature warping for acceleration. They divided frames into two types, key frames and non-key frames. Key frames are sent to the CNN for segmentation, while non-key frame results are obtained by warping. Recently, Hu~et al.~\citep{hu2020temporally} proposed to approximate high-level features by composing features from several shallower layers.
		% problems 1. bias, 2. acumulate  equation
		% bias, key-frame selection
		These warping-based approaches efficiently speed up the inference phase since the computational cost of warping is much less than that of CNN. However, both the accuracy and robustness of these methods deteriorate due to the following reasons. First, neither optical flows nor motion vectors can estimate the precise motion of all pixels. Thus, there always exist unavoidable biases~(errors) between the warped features and our expected ones. Second, in the case of consecutive non-key frames, the errors accumulate fast, leading to unusable results.
		To address the error accumulation problem, Li~et al.~\citep{low-latency} and Xu~et al.~\citep{dvsnet} proposed to adaptively select key frames by predicting the confidence score for each frame. Jain~et al.~\citep{jain2018fast} introduced bi-directional features warping to improve accuracy. However, all these approaches lack the ability to correct warped features.
		
		% Ours
		%The main difference between the proposed Warp-Refine Network and previous warping-based methods is that our approach firstly includes the refinement stage after feature warping.


		% Our approach is related to motion compensation in two folds
			% warping
			% refine <-> residual in 
		%Our WRNet is related to motion compensation in the following aspects. First, the feature warping is similar with warping for images. Second, inspired by the correction step in motion compensation, we propose the context feature refinement~(CFR) module to perform correction in feature space. Last, observing the spatial consistency between image space and feature space, we propose to use the residual map in image space to guide the learning of CFR.

		 
		
		

